Managing Recurrent Virtual Network Updates in Multi-Tenant Datacenters: A System Perspective

With the advent of software-defined networking, network configuration through programmable interfaces becomes practical, leading to various on-demand opportunities for network routing update in multi-tenant datacenters, where tenants have diverse requirements on network routings such as short latency, low path inflation, large bandwidth, high reliability, etc. Conventional solutions that rely on topology search coupled with an objective function https:// www.overleaf.com/project/5beb742041ab9c0e3caec84f to find desired routings have at least two shortcomings: (i) they run into scalability issues when handling consistent and frequent routing updates and (ii) they restrict the flexibility and capability to satisfy various routing requirements. To address these issues, this paper proposes a novel search and optimization decoupled design, which not only saves considerable topology search costs via search result reuse, but also avoids possible sub-optimality in greedy routing search algorithms by making decisions based on the global view of all possible routings. We implement a prototype of our proposed system, OpReduce, and perform extensive evaluations to validate its design goals.

==> Managing Recurrent Virtual Network Updates in Multi-Tenant Datacenters A System Perspective/background.tex <==
\section{Background and Motivation}\label{sec:background}
\subsection{Managing Per-Tenant Routing}\label{sec:routing_control}
%assumes that multi-tenant data center operators have incentives to
%manage network traffic at the granularity of individual tenants. We are not
%claiming that per-tenant routing control is necessarily the optimal choice in
%multi-tenant data center designs, but we would like to explain that it
%is indeed a desirable feature for network operators. 
%In this section, we explain why in-network routing control at the granularity of tenant is the right design philosophy in multi-tenant data centers. 


%Virtualization and multi-tenancy creates unique and challenging networking
%environment. Specifically, computational resources in data centers are
%virtualized into VMs~\cite{vmware}. Tenants who purchase the computational
%resources get a set of VMs, which are re typically hosted by several physical
%servers due to resource limitations and constraints on one single host. To
%ensure tenant isolation and give full networking flexibility for each tenant,
%such as having self-defined addresses, the host hypervisors create a
%virtualization layer~\cite{openvswitch} between the VMs and hosts. Thus, to
%support the communication among the VMs in one tenant, the source host
%hypervisor first encapsulates the VM traffic using its own addresses and
%\emph{tunnels} the traffic to the destination host, whose hypervisor
%decapsulates the packets and deliver them to the VMs~\cite{vmware, vl2,
%netlord, secondnet}

For configuration simplicity, encapsulations protocols such as
VXLAN~\cite{vxlan} and NVGRE~\cite{nvgre} are widely adopted 
in cloud~\cite{vmware}. However, by simply tunneling tenant traffic, 
network operators lose the traffic visibility and accountability, \ie they 
are not able to identify the origin of network traffic since packets are sent 
on behalf of hypervisors and one hypervisor may host VMs for multiple tenants. 
Such invisibility becomes even worse when datacenters run link aggregation
and/or perform load balancing (\ie ECMP, Hedera~\cite{hedera}, or CONGA~\cite{conga}) 
to spread traffic across redundant physical links. As a result, even if
one tenant occupies only a small fraction of computation resources 
in the datacenter, %(\eg a few VMs hosted by a small number of hypervisors, 
its traffic could appear on many physical links, making network operators 
unaware of actual in-network traffic forwarding for the tenant. 

%The lack of the in-network routing management at the granularity of tenant creates
The lack of in-network tenant-routing management causes various
operation restrictions. For instance, it is difficult for network operators to
perform monitoring, measurement and trouble-shooting for a tenant as
its traffic may spread across many network links.
%These management restrictions further result in networking performance degradation. 
%For example, when encountered with link congestion or failures, it is difficult for network operators to 
%locate affected tenants and reconfigure their networks in time. 
%Moreover, performance-oriented virtual network embeddings such as 
%bandwidth guarantee embeddings~\cite{predictable,secondnet} 
%cannot be easily enforced due to the lack of tenant-level routing control. 
Further, as virtual private cloud gains popularity, more tenants have 
incentives to customize their private cloud based on their own needs, \eg 
one tenant may want to promote latency performance of web servers,  
whereas someone else may want to optimize bandwidth for
MapReduce tasks. Without explicit tenant-level 
routing control, it is difficult to customize routings for
individual tenants.

Thus, it is desirable for network operators to have explicit control over tenant routings. In particular, for each
tenant, network operators explicitly configure a Virtual Tenant Network
(VTN), which is an overlay network connecting
the tenant's VMs. The tenant's traffic is confined within its VTN and no other physical links 
besides the ones in its VTN can carry the tenant's traffic. 
As tenants can be identified by their VTNs, traffic is accountable, 
which eliminates these management limitations. 
Further, network operators can customize a tenant's routing based on its 
requirement by embedding its VTN into an overlay that can best satisfy the 
requirement. 

The traditional way of embedding VTN for a tenant relies on topology search 
coupled with an objective function to find the desired overlay. 
Such an approach, however, has at least two shortcomings: \first it runs into scalability 
issues when handling frequent VTN embedding requests and \second it may 
be insufficient to find the optimal overlay for complex embedding goals.
Next, we elaborate on the two issues. 

\subsection{Frequent VTN Updating Requests}\label{sec:all_time}
In production multi-tenant datacenters, managing VTN embeddings/updates are all-time tasks on the basis
of individual tenants, which are up to tens of thousands~\cite{amazon_dc_size}. 
%One VTN embedding is about first searching an 
%overlay network and then configuring the switches on the overlay for the tenant. 
%Although how to perform one-time VTN embedding might be
%intuitive, consistently and frequently
%performing significant amounts of embedding tasks faces scalability concerns.
%In multi-tenant data centers, 
VTN embedding requests are triggered by many sources including 
network load dynamics, link congestions and failures, hot spots, 
tenant departures and so on. 
Although efficient graph search algorithms, such as Prim's and
Kruskal's, have been proposed for decades, consistently and frequently
performing overlay search in large topology for a large number of VTN updates still 
imposes significant cost. Resolving the scalability problem 
is the first step towards efficient tenant-routing management. 


\subsection{Fulfilling VTN Embedding Goals}\label{sec:embedding_goal}
A VTN embedding/update is as simple as finding a random overlay 
network for the tenant. Instead, the VTN may need to satisfy various 
requirements such as guaranteed bandwidth~\cite{predictable,secondnet,tag},  
bounded latency~\cite{silo,qjump}, required security appliances
~\cite{cloudwatcher,netsecvisor}, and other performance metrics 
depending on the tenant's SLA. As these embedding goals become more complex, 
it is uncertain that the conventional search \& optimization coupled solution can find 
the real optimal routing. 

\iffalse
both network operators and tenants hope to 
%determine the most desired one among all possible choices so as to 
achieve certain networking objectives during VTN embeddings. 
For instance, previously proposed bandwidth guarantee embedding~\cite{predictable,secondnet} is one kind of 
performance-oriented virtual network embeddings. 
The traditional way of achieving embedding goals relies on a well-designed topology search algorithm to 
find the desired overlay network. 
For example, the Prim's and Kruskal's minimum spanning tree algorithms 
can be used to find an overlay with smallest number of hops~\cite{kruskals,prims}. 
Moreover, in order to make search process efficient, the algorithm is typically designed to be greedy 
so as to reduce search space in each iteration. 

However, as embedding goals are more complicated, search algorithms may fall short to achieve these 
goals. For instance, one embedding requirement considering multiple performance metrics (\eg bandwidth, latency and 
security features) cannot to be easily fulfilled by a search algorithm. 
Furthermore, due to the virtualization of computation resources (\ie tenants are assigned VMs rather than 
servers), we find that search algorithms may fail to determine the most desired overlay even for simple embedding 
goals. 
\fi

We use an illustrative example in Figure~\ref{fig:mst} to demonstrate such sub-optimality. 
Network operators perform VTN update for a tenant whose VMs are hosted by the set of 
hypervisors $[\textsf{S}_\textsf{1}, \textsf{S}_\textsf{2}, \textsf{S}_\textsf{3}]$. 
The embedding goal is to minimize the communication cost of all virtual links. 
For simplicity, we define the communication cost of a virtual link as  
the number of hops on the path connecting the two VMs of the virtual link. 
Thus, if VM1 and VM2 take path 
$\textsf{S}_\textsf{1}\textsf{-}\textsf{A}\textsf{-}\textsf{C}\textsf{-}\textsf{S}_\textsf{2}$,
the cost is 3. 

This embedding is a classic minimum spanning tree problem that can  
be solved by a greedy topology search algorithm. %coupled with an objective function. 
At certain intermediate state of the overlay search (Figure \ref{fig:mst}(a)), 
\textsf{AB} has been appended to the overlay. Based on the tie breaker in the algorithm, 
\textsf{BC} is then appended to the ongoing
overlay, and the final overlay returned by the algorithm is $\textsf{S}_\textsf{1}\textsf{-A}$, 
$\textsf{S}_\textsf{2}\textsf{-C}$, $\textsf{S}_\textsf{3}\textsf{-B}$, 
\textsf{AB}, \textsf{BC} (Figure \ref{fig:mst}(b)). With a different algorithm, 
\textsf{AC} could be the link to append after state (a) rather than \textsf{BC}, and the 
final overlay returned will the one shown in Figure \ref{fig:mst}(c). 
%$\texttt{S}_\texttt{1}\texttt{-A}$, 
%$\texttt{S}_\texttt{2}\texttt{-C}$, $\texttt{S}_\texttt{3}\texttt{-B}$,
%\texttt{AB}, \texttt{AC} (Figure \ref{fig:mst}(c)). 
However, no matter how the search algorithm is designed, 
the optimality of an overlay is up to the distribution of VMs. 
Although VM locations are known a priori, in an intermediate state, 
the search algorithm cannot determine exactly which virtual links a physical link 
will carry. Thus, the search algorithm cannot guarantee to capture the real optimal 
overlay (Figure \ref{fig:mst}(d)). In fact, due to the lack of mapping between virtual links and physical links, 
the conventional search \& optimization coupled solution is subject to  
sub-optimality when optimizing any performance metric involving virtual links. 

\emph{We note that providing rigid theoretical proof to show the sub-optimality of 
	 the conventional search \& optimization approach is beyond the scope 
	 of this paper. Instead, this paper focuses on offering a system perspective 
	 of how tenant routings are managed in practice, especially based on our experience with 
	 production datacenters.} 


\subsection{Decoupling Search and Optimization}\label{sec:decouple}
To address the above challenges, \sys proposes a search and optimization 
decoupled design. For a routing update request, \sys first comprehensively finds all 
desired overlay candidates considering only VM locations. Then it applies 
an objective function, designed with the global view on all routing candidates, 
to finalize the optimal one. In the above example, \sys will first obtain all 3 
overlay candidates (figures (b), (c) and (d) in Figure~\ref{fig:mst}) and 
then evaluate them to find the optimal one (Figure \ref{fig:mst}(d)). With the global view 
on all candidates, \sys knows the exact mapping between virtual links 
and physical links. Thus, it can design a global objective function in evaluation to 
guarantee optimality. Further, as topology search is not directed by any objective 
function, search results are general so that they can be reused for further VTN updates that 
have the same VM locations. This saves considerable cost for performing 
frequent VTN updates in large scale datacenters. 

\iffalse
To allow complete flexibility and capability to fulfill embedding goals as well 
as saving considerable topology search efforts. Specifically, \sys comprehensively finds a list of desired 
overlay candidates simply based on VM location and network topology, then it  
determines the most desired candidate afterward to embed a tenant. 
Under such a design, network operators will first obtain three overlay candidates 
(Figure \ref{fig:mst}(b), (c) and (d)) in the previous 
example and then evaluate them to finalize the best one (Figure \ref{fig:mst}(d)). 
As network operators now know the exact path used by each VM pair communication in each candidate, 
they can accurately evaluate these overlays. 
In fact, regardless of how complicated and sophisticated the embedding goal is, 
network operators are no longer restricted to search algorithms 
to achieve the goal. Instead, they already have all desired candidates in the first place so that 
they are completely free to design arbitrary algorithms to determine the best one.  
Furthermore, the decoupled design eliminates topology search cost for a considerable 
fraction VTN embedding requests: all VTN embeddings  for new tenants whose VM locations have been explored and 
all VTN re-embeddings for existing tenants due to network dynamics or new embedding goals. 
\fi


%\subsection{Embedding Virtual Tenant Networks}\label{sec:vm_place}
%Most VTN embedding solutions consider VM placement and VTN embedding together
%as one problem~\cite{secondnet}. However, in practice, where to place VMs and how to
%embed VTNs based on the given VM locations are usually separated
%issues. Specifically, VM placement is constrained by
%other factors besides networking performance in practice. For instance, 
%VM placement is often restricted by the available resources (\eg
%memory, storage, CPU) one hypervisor has and what type of VMs one hypervisor can host (\eg 
%some hypervisors are dedicated for computation intensive VMs).  
%After VM locations are decided, it is the turn for network
%operators to determine the best networking configuration to fulfill the tenant's networking
%requirements. 

%\sys's focus is on the problem of embedding VTN after VM locations are
%determined, but note that \sys is not restricted by the fact. 


%To begin with, \sys accepts the input as a tenant's VM placement, which is defined as the set of physical servers hosting the tenant's VMs (\eg in Figure \ref{fig:mst}, the tenant's VM placement is $[S1,S2,S3]$). Note that we decouples VM placement and network optimization is not due to any limitation of \sys. This is because in reality VM placement is often constrained by other factors besides networking performance. Specifically, on the one side, operators have the incentive to keep the VMs belonging to one tenant local to reduce their consumption of networking resources since communication among VMs located within one hypervisor can be finished within the same host. On the other side, VMs fragmentarily distribute across multiple hypervisors are common because hypervisors have the constraints on the maximum number of VMs and the type of VMs they can host (\eg some hypervisors are dedicated for computation-oriented VMs). Therefore, we can expect that each tenant's VMs often span across a few hypervisors (\eg less than $5$) whereas the exact VM placement cannot be directed by networking optimization. 
 



==> Managing Recurrent Virtual Network Updates in Multi-Tenant Datacenters A System Perspective/conclude.tex <==
\section{Conclusion}
\label{sec:conclude}
In this paper, we present \sys, a system for managing virtual tenant 
network update in multi-tenant datacenters. 
Conventional solutions that rely on topology search coupled with an objective function 
to find desired routings have at least two shortcomings: scalability 
issue for handling recurrent routing updates and the inefficiency 
for satisfying various routing requirements. To address these issues, 
\sys proposes a novel search and optimization decoupled design, which enables 
routing search result reuse and guaranteed routing optimality. We implement 
a prototype of \sys and perform extensive evaluations to valid \sys's design goals. 
Evaluation results show that \first Even for complex VTN embedding goals, 
\sys ensures routing optimality which yields significant networking performance improvement 
over conventional approaches; \second \sys greatly reduces search cost for managing 
numerous routing updates and imposes small system overhead. 


\iffalse
In this paper, we present the design, implementation and evaluation of \sys, a  
system for automating virtual tenant network management in multi-tenant data centers.
\sys's in-network routing control and the novel decoupled search and embedding design offer 
both management benefits and performance improvement. For instance, 
with explicit tenant routing control, \sys allows network operators to perform efficient tenant network management such as monitoring 
and trouble shooting, and customizes tenants' routings based on their requirements. 
Furthermore, the decoupled design enables network operators to have complete 
flexibility and capability to fulfill arbitrary VTN embedding goals, which will 
improve a wide range of networking performance (\eg up to $5\times$ better flow completion times in our evaluation). 
Based on our hands on experience with the physical testbed and 
system evaluation, we demonstrate that \sys can scale to manage large scale multi-tenant data centers. 
\fi



==> Managing Recurrent Virtual Network Updates in Multi-Tenant Datacenters A System Perspective/evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}
Our evaluation centers around the followings. \first In \S \ref{sec:congestion_aware}, we show  
%the inefficiency of conventional search \& optimization coupled solution, and show that 
\sys is guaranteed to find the least congested routings for VTN embeddings under various 
settings, which yields significant networking performance 
improvement over common practice. \second In \S \ref{sec:system_evaluation}, 
we show that \sys greatly reduces the search cost for managing numerous routing updates 
and imposes small system overhead while managing routing updates in large scale datacenters. 


\subsection{Congestion-Aware Routing Updates}\label{sec:congestion_aware}
One representative goal for routing updates in multi-tenant datacenters is to find 
the least congested routing to re-accommodate a tenant. The traditional search \& 
optimization coupled solution for finding the desired routing is using the 
Prim's minimal spanning tree algorithm with physical link utilization as the edge weight. 
However, since network traffic is generated by 
VM pairs, minimizing the congestion experienced by virtual 
links is the more direct and therefore more accurate goal for finding the least congested routing. 
Thus, \sys uses the following algorithm to determine the most desired routing. 
Assume \sys produces $m$ routing candidates $\{\mathcal{T}_1,...,\mathcal{T}_m\}$ for 
a routing update request that has $n$ virtual links $\{l_1,...,l_n\}$. 
Then the most desired routing is 

\begin{equation}\label{eqn:routing}
\mathcal{T}^* = \min_{\mathcal{T}_k} \frac{\sum_{i=1}^n ~ \lambda_i\cdot \mathcal{F}_k(l_i)}{n},
\end{equation}
where $k\in[1,m]$, $\mathcal{F}_k(l_i)$ is the congestion level experienced by virtual link $l_i$ 
in routing candidate $\mathcal{T}_k$ and $\lambda_i$ is the weight of $l_i$. 
In \sys's instance deployed in our production datacenters, both $\mathcal{F}$ and $\lambda_i$ 
are configurable to enable highly flexible routing customization. 
For evaluation purpose in this paper, $\mathcal{F}_k(l_i)$ is 
defined as the highest congestion level of all physical links in $\mathcal{T}_k$ that carry $l_i$, 
where the congestion level of a physical link is estimated as its average link utilization. 
Further, all virtual links are equally weighted. 

Besides the conventional search \& optimization coupled solution (referred to as the \emph{local} solution), 
we also compare \sys with flow-level ECMP, the common practice for load balancing 
and congestion reduction in datacenters, and the \emph{bottomline} solution which 
embeds VTN to a randomly selected routing candidate. 

For each embedding request, we compare the routing determined by \sys and the ones
selected by the other three solutions. We use average flow completion time (FCT) 
as the metric to quantify the congestion experienced by virtual links
(similar to~\cite{why_fct, conga}), expecting that a better routing 
will have shorter average FCT. \emph{Note that we do not claim that FCT is either the only or 
the optimal metric. We use FCT for the sake of quantifiable results.}

\begin{figure}[t]
	\centering
	\mbox{
		\subfigure[\label{fig:flow:a}\small Enterprise workload\cite{conga}]{\includegraphics[scale=0.35]{Figures/flow_dis1.pdf}}  
		\subfigure[\label{fig:flow:b}\small Data-mining workload\cite{vl2}]{\includegraphics[scale=0.35]{Figures/flow_dis2.pdf}} 
	}
	\caption{Empirical workloads used in evaluation.
		%representing a large enterprise data center
		%workload. The cloud cluster workload is from VL2, a large cluster providing
		%cloud services~\cite{vl2}. 
	}
	\label{fig:flow}
\end{figure}

\begin{figure}[t]
	\centering
	\mbox{
		\subfigure[\small Background utilization in one snapshot\label{fig:fct_back}]{\includegraphics[scale=0.26]{Figures/testbed_util.pdf}}
		\subfigure[\small Desired routings produced by each solution\label{fig:fct_one_trial}]{\includegraphics[scale=0.26]{Figures/testbed_embed.pdf}}
	}
	\mbox{
		\subfigure[\small Average FCT in each experiment set \label{fig:fct_all_trial}]{\includegraphics[scale=0.42]{Figures/testbed_congestion_aware_embed.pdf}}
	}
	\caption{Testbed experiments for improving FCTs.}
	\label{fig:testbed_CA}
\end{figure}

\begin{figure*}[t]
	\centering
	\mbox{
		\subfigure[\small FCT min-mean-max distribution.\label{fig:baseline:a}]{\includegraphics[scale=0.48]{Figures/congestion_aware_baseline_cdf1_new.pdf}}
		\subfigure[\small False rate.\label{fig:baseline:b}]{\includegraphics[scale=0.48]{Figures/congestion_aware_baseline_cdf1_diff_RR.pdf}}\quad
		\subfigure[\small FCT min-mean-max distribution.\label{fig:baseline:c}]{\includegraphics[scale=0.48]{Figures/congestion_aware_baseline_cdf2_new.pdf}}
		\subfigure[\small False rate.\label{fig:baseline:d}]{\includegraphics[scale=0.48]{Figures/congestion_aware_baseline_cdf2_diff_RR.pdf}}
	}
	\caption{Impact of the fabric load on \sys's performance.
		The normalized FCT is used as the performance metric. 
		%The smaller the normalized FCT means the higher FCT reduction, \ie the more efficient resource utilization. 
		Part (a) and (b) use the enterprise workload~\cite{conga}. Part (c) and (d) use the data-mining workload~\cite{vl2}.
	}
	\label{fig:baseline}
\end{figure*}

\subsubsection{Testbed Experiments}
We start the evaluation on our physical testbed. 
We build a network topology illustrated in Figure \ref{fig:fct_back}. 
The datacenter has pre-embedded tenants to generate traffic 
using our client/server programs. The clients initiate long-lived TCP connections to 
randomly selected servers to request flow transfers.  All VMs run both the client and 
server programs. Only intra-tenant communication is allowed. 

In this experiment, we perform routing update for a tenant who has 10 VMs 
that are randomly distributed in all four hypervisors on our testbed. 
In total, we perform $40$ sets of experiments under different network utilization. 
Figure \ref{fig:fct_back} shows the snapshot of network utilization 
in one experiment set. In each experiment set, we perform $3$ individual routing updates 
using \sys, ECMP and the bottomline solution. 
After the tenant VTN is embedded, its virtual links (VM pairs) start to 
generate traffic using our client/server programs. Flow sizes are randomly 
sampled from the empirical datacenter workload~\cite{conga}. To 
ensure fair comparison, the set of flow sizes used for the 3 experiments in each  
experiment set is identical. We compute the average FCT 
among all flow transfers as our performance metric. 

Figure \ref{fig:fct_one_trial} illustrates the desired routing produced by each solution 
for the network utilization shown in Figure~\ref{fig:fct_back}. 
Since \sys first outputs all routing candidates (\ie 
$\textsf{E}_\textsf{1}\textsf{-}\textsf{C}_\textsf{1}\textsf{-}\textsf{E}_\textsf{2}$, 
$\textsf{E}_\textsf{1}\textsf{-}\textsf{C}_\textsf{2}\textsf{-}\textsf{E}_\textsf{2}$, 
$\textsf{E}_\textsf{1}\textsf{-}\textsf{C}_\textsf{3}\textsf{-}\textsf{E}_\textsf{2}$) and 
then applies the objective function (Equation~(\ref{eqn:routing})) to determine the most desired one, it can 
always find the least congested routing ($\textsf{E}_\textsf{1}\textsf{-}\textsf{C}_\textsf{1}\textsf{-}\textsf{E}_\textsf{2}$ 
in this case). However, both ECMP and bottomline are unaware of the link utilization. 
Consequently, their static hashing could result in overwhelming these more congested links.  

Figure \ref{fig:fct_all_trial} plots the average FCT 
in each experiment set when using enterprise workload~\cite{conga} 
(results for using data-mining workload~\cite{vl2} are similar, and we omit them for brevity).  
Although the bottomline solution and ECMP may produce different FCTs in one set, 
their average FCTs over all sets are close. 
Comparing with these two solutions, \sys can consistently find the 
optimal routing, yielding ${\sim}30$\% less FCTs on average and up to 
${\sim}5$x reduced FCTs in some sets (outside the plot scope of Figure \ref{fig:fct_all_trial}). 

Note we do not compare \sys with the local solution in our testbed experiments. This is because 
the local solution and \sys will produce the same routing in such a small topology. Next 
we show that given large network topologies, it is very likely for the local solution 
to return sub-optimal overlays, which results in significant performance degradation.



\subsubsection{Large Scale Simulations}
\begin{table}
	\centering
	\resizebox{0.95\linewidth}{!}{%
		\begin{tabular}{| c  || c || c || c || c || c |}
			\hline
			\begin{tabular}[c]{@{}l@{}} Exp.\\ NO. \end{tabular} & 
			Topology & 
			{\begin{tabular}[c]{@{}l@{}} Fabric\\~~load \end{tabular}} & 
			{Workload} & 
			{\begin{tabular}[c]{@{}l@{}} ~~\# VMs\\ per tenant \end{tabular}} & 
			{\begin{tabular}[c]{@{}l@{}} ~~Average\\ VTN scale \end{tabular}}  \\
			\hline
			1 & $k{=}8$ FT & * & enterprise & 20 & 4 \\
			\hline
			2 & $k{=}8$ FT & $3{:}1$ & * & 20 & 4 \\
			\hline
			3 & * & $3{:}1$ & enterprise & 20 & 4 \\
			\hline
			4 & $k{=}8$ FT & $3{:}1$ & enterprise & 20 & * \\
			\hline
			5 & $k{=}8$ FT & $3{:}1$ & enterprise & * & 4 \\
			\hline
	\end{tabular}}
	\caption{Experimental settings. 
		%for \sys's performance evaluation. 
		``*'' refers to that we vary the factor to isolate its impact in the experiment. 
		%The value of
		%each factor, when we randomize a VTN request, is a Guasian distribution function
		%whose expected value is listed in the table, e.g., in exp NO. 1's, the number of
		%VMs in a VTN request is a randomized number around 10.
	}\label{tab:setting}
\end{table}




In order to investigate how \sys's performance is affected by various
factors that are not covered by our small-scale testbed experiments, 
we perform detailed simulations using large scale 
datacenter topologies and empirical workloads obtained 
from production datacenters (Figure \ref{fig:flow}). 
As summarized in Table~\ref{tab:setting},
we thoroughly evaluate the performance of \sys under the 
impact of five factors: the topology, the
network/fabric load, the traffic workload, the average number of VMs 
occupied by a tenant, and the average VTN scale.


\iffalse
%We consider four large scale data center topologies (Clos with $2{:}1$ over-subscription ratio, $k{=}8$
%and $k{=}16$ fat-tree and an organized topology with random ``short-cut" links).
%As background data center utilization is needed, 
To create background datacenter utilization for our evaluation, 
we first create an empty datacenter and then embed $\lambda$
tenants using \sys. We also try other solutions for background 
tenant embedding. Consider the first $\lambda$ embedded VTNs as the background, we embed a new
VTN using different solutions among \sys, the bottomline, the local
and ECMP. Through varying $\lambda$, we can create different loads in the data
center fabric and fairly compare different solutions. 
\fi

\noindent\textbf{Various Fabric Loads (Exp NO. 1):} 
In multi-tenant datacenters, fabric load can be quantified as the VM over-subscription ratio, which is defined as 
the ratio of worst-case achievable aggregate bandwidth among VM pairs 
to the total capacity of the topology. A fat-tree fabric 
has an hypervisor over-subscription of $1{:}1$ because all hypervisors may potentially send at 
the full bandwidth of their network interfaces. Thus, if the average number of 
VMs hosted by a hypervisor is $N$, the VM over-subscription ratio is $N{:}1$. 
Hereafter, we use the VM over-subscription ratio as \emph{load degree}.

We tune the datacenter load degree in the range of $1{:}1$-$7{:}1$ by varying the
number of embedded tenants. For each load, we 
create $5$ different snapshots to avoid bias. 
For each snapshot, we randomly pick a tenant to perform routing update 
using all four solutions: \sys, the local solution, ECMP and the bottomline solution. 
Thus, we perform $4$ independent experiments for the tenant. 
In each solution, after the desired routing is finalized, 
we assign each virtual link a randomly sampled flow size 
to generate traffic and compute the average FCT among all flow transfers. 
Among all $4$ experiments for the same tenant, we use the same set of flow sizes.  
After finishing the current tenant, we recover the network snapshot and re-sample 
another tenant to continue evaluation. In total, 100 routing updates are performed 
for each snapshot. 

Figure \ref{fig:baseline} plots the min-median-max distribution of the
averaged FCT across all $5$ snapshots for each load degree. 
As illustrated in the Figure \ref{fig:baseline:a}, \sys significantly outperforms 
ECMP and bottomline: up to 80\% FCT reduction for small fabric loads and at least $40$\% 
FCT reduction for all loads. Again, this is because ECMP and bottomline are static
solutions that are unaware of the network utilization. Further, 
as load degree increases, \sys offers less FCT reductions since 
there is less routing optimization space in heavily utilized network. 
Since production datacenters are typically over-provisioned, 
we can expect large performance benefits offered by \sys in production datacenters. 


Due to the lack of exact mapping between virtual links and physical links, 
the local solution often produces sub-optimal routings. As shown in Figure \ref{fig:baseline:b},  
with high probabilities (up to ${\sim}60$\%), the local solution returns an overlay 
different from the one produced by \sys. Consequently, these sub-optimal 
routings result in $1.2{-}4$x FCT inflation, compared with 
the routings produced by \sys (Figure \ref{fig:baseline:a}).

\noindent\textbf{Datacenter Traffic Workload (Exp NO. 2)}: 
In Figures \ref{fig:baseline:a} and \ref{fig:baseline:b}, we use the enterprise datacenter workload. We repeat the 
same experiment using the data-mining workload to learn the impact of traffic workload on \sys's performance. 
The results, plotted in Figures \ref{fig:baseline:c} and \ref{fig:baseline:d}, show that \sys provide similar benefits for 
data-mining workload. 

\noindent\textbf{Fabric topologies (Exp NO. 3):} 
We investigate four datacenter topologies: three organized topologies (Clos, $k{=}8$ and $k{=}16$
fat-tree) and another organized topology added with random short-cuts. 
%Among the three organized topologies, 
The Clos topology has the same number of hypervisors as the $k{=}8$ fat-tree topology except that the 
over-subscription ratio is $2{:}1$. All three organized topologies have different 
routing redundancy. In particular, they have $8$, $16$ and $64$ shortest paths 
between two randomly chosen hypervisors in different pods, respectively. 
The short-cut topology is built 
by adding random links into the $k{=}8$ fat-tree topology. The links are randomly 
added between ToR switches to inter-connect different pods so that 
besides traversing through the core switches, 
the inter-pod communication can alternatively use the short-cut bridges 
as well. We set the load degree as $3{:}1$ in all these topologies.  
%as production data centers often have around $3\times$ over-provisioning. 

\begin{figure}[t]
  \centering
  \mbox{
    \subfigure{\includegraphics[scale=0.55]{Figures/congestion_aware_baseline_topology_layer.pdf}}
    }
  \caption{Impact of datacenter topology on \sys's performance of FCT reduction.
  %The more link redundancy in a topology, the higher FCT reduction.
  % for \sys.
  %meaning the better resource efficiency. 
  }
  \label{fig:topology}
\end{figure}

%To evaluate the impact of topology, we investigate how the
%topology affects \sys's performance in FCT
%reduction compared with the bottomline. 
For each topology, we perform the similar experiments as in evaluating the
impact of fabric loads. Figure \ref{fig:topology} plots the CDF of all obtained FCT 
reductions (compared with the bottomline solution). 
By comparing the results of all 3 fat-tree topologies, we conclude  
that \sys offers more benefits for topologies built with more redundant links.  
This is because \sys has larger optimization space in more redundant topologies. 

We further investigate how topology short-cuts may affect the performance of \sys. 
In organized datacenter topologies, alternative routing options typically have 
less diversity in the sense that they all have the same number of hops, 
%\eg $\texttt{E}_\texttt{1}\texttt{-}\texttt{C}_\texttt{1}\texttt{-}\texttt{E}_\texttt{2}$, 
%$\texttt{E}_\texttt{1}\texttt{-}\texttt{C}_\texttt{2}\texttt{-}\texttt{E}_\texttt{2}$ and
%$\texttt{E}_\texttt{1}\texttt{-}\texttt{C}_\texttt{3}\texttt{-}\texttt{E}_\texttt{2}$ 
%in Figure~\ref{fig:fct_back}, 
although they are varying in terms of utilization. In contrast, short-cut topology can 
create more diverse routings with different numbers of hops as well as different utilization. 
Thus, \sys has even larger optimization space in the short-cut topology 
so as to produce more performance benefits. 

\begin{figure}[t]
  \centering
  \mbox{
    %\subfigure{\includegraphics[scale=0.55]{Figures/congestion_aware_baseline_diff_hyper_ecmp_global.pdf}}
    \subfigure[\label{fig:vtn_scale}Average VTN scale (Exp NO. 4)]{\includegraphics[scale=0.38]{Figures/congestion_aware_VTN_scale.pdf}}
}
\mbox{
    \subfigure[\label{fig:vm_size}Average per-tenant VM count (Exp NO. 5)]{\includegraphics[scale=0.38]{Figures/congestion_aware_diff_VM.pdf}}
  }
  \caption{\sys offers consistent benefits for different VTN scales and different per-tenant VM counts.}
  \label{fig:4and5}
\end{figure}

\iffalse
\begin{figure}[t]
  \centering
  \mbox{
    \subfigure{\includegraphics[scale=0.55]{Figures/congestion_aware_baseline_diff_VM.pdf}}
  }
  \caption{Impact of the average \# of VMs per VTN on \sys's performance of FCT
  reduction. The \# of VMs has negligible impact on \sys's performance.}
  \label{fig:VM_count}
\end{figure}
\fi


We also investigate the average VTN scale $\mathcal{N}_h$ (the average number of hypervisors 
used by a tenant's VMs) and the average per-tenant VM count $\mathcal{N}_v$. 
We consider $\mathcal{N}_h{=}[3,4,5]$ and $\mathcal{N}_v{=}[10,20,30]$ 
since they are the common cases in our production datacenters. 
We find that \sys consistently provides performance benefits in these settings 
(Figure~\ref{fig:4and5}).

%\noindent\textbf{VTN scale (Exp NO. 4):} The VTN scale of a
%tenant is defined as the number of the hypervisors $\mathcal{N}_h$ that its VMs are spanning across. 
%We consider $\mathcal{N}_h{=}2,3$ and $4$ in our experiments since they are 
%the common practices, \ie operators often enforce a maximum number of
%hypervisors to confine the scale of the VTN. 
%The results (Figure \ref{fig:VTN_size}) show that 
%\sys's FCT reduction has a larger margin 
%for a smaller VTN size because the traffic of 
%tenants with smaller VTN sizes concentrates on smaller numbers of links so 
%that the hashing collision overwhelms certain links to a larger extent. 
 
%\noindent\textbf{VM number per-tenant (Exp NO. 5):} The number of VMs occupied by 
%each tenant $\mathcal{N}_v$ determines the number of virtual links of 
%each tenant. We consider $\mathcal{N}_v{=}10, 15$ and $20$ in our evaluation. 
%The results (Figure \ref{fig:VM_count}) show that \sys provides consistent 
%benefits no matter how many are VMs owned by each tenant.

%To sum up, as long as the data centers have 
%optimization space (\eg redundant routings and reasonable over-subscription ratios), 
%\sys consistently offers significant networking performance benefits. 
%without further requirements for tenants (\eg the VTN scale and the number of VMs occupied by one tenant). 

\iffalse
\subsection{Fulfilling Bandwidth Requirements}\label{sec:bandwidth}
In \S\ref{sec:FCT}, we investigate the benefits that
\sys can bring to network operators in allocating resource across tenants. From a
single tenant's perspective, the tenant may have the incentives to explicitly express the
resource requirements and expect the network operators to be able to fulfill
them. For instance, a tenant network running MapReduce jobs may require 
larger bandwidth for its virtual links since many-to-many data shuffles between the 
map and reduce stages occupy large bandwidth and often consume non-trivial time~\cite{shuffle}. 
%To fulfill such a requirement, \sys allows 
%network operators to speed up data shuffles via explicit 
%tenant routing control. Specifically, they can simply embed the 
%tenant into the routing with the most available bandwidth. Further, 
%network operators can re-embed some of existing VTNs to ``make more
%room'' for the new embedding request without downgrading existing VTNs' performance. 



%\noindent\textbf{Shuffle speed up:} To embed the new tenant network, \sys outputs $3$ virtual network candidates based on the topology: $\texttt{H}_\texttt{1}\texttt{-E}_\texttt{1}\texttt{-C}_\texttt{1}\texttt{-E}_\texttt{2}\texttt{-H}_\texttt{3}$, $\texttt{H}_\texttt{1}\texttt{-E}_\texttt{1}\texttt{-C}_\texttt{2}\texttt{-E}_\texttt{2}\texttt{-H}_\texttt{3}$ and $\texttt{H}_\texttt{1}\texttt{-E}_\texttt{1}\texttt{-C}_\texttt{3}\texttt{-E}_\texttt{2}\texttt{-H}_\texttt{3}$. Via explicit tenant-level routing control, network operators can embed the tenant network into $\texttt{H}_\texttt{1}\texttt{-E}_\texttt{1}\texttt{-C}_\texttt{1}\texttt{-E}_\texttt{2}\texttt{-H}_\texttt{3}$, which has the largest available bisection bandwidth among all the candidates (Figure \ref{fig:topology:util}). Furthermore, they can reshape the network utilization by shifting the traffic from core switch $\texttt{C}_\texttt{1}$ to $\texttt{C}_\texttt{2}$, who has enough capacity to hold the new traffic. Thus the data shuffle is further speeded up via the newly updated $\texttt{H}_\texttt{1}\texttt{-E}_\texttt{1}\texttt{-C}_\texttt{1}\texttt{-E}_\texttt{2}\texttt{-H}_\texttt{3}$. Note that, without VM migration, we cannot shift all traffic so that $\texttt{H}_\texttt{1}\texttt{-E}_\texttt{1}\texttt{-C}_\texttt{1}\texttt{-E}_\texttt{2}\texttt{-H}_\texttt{3}$ has almost zero utilization. This is because the background tenants whose VMs are placed in $\texttt{H}_\texttt{1}$ and $\texttt{H}_\texttt{3}$ consume the bandwidth as well. Figure \ref{fig:shuffle:a} shows that with background VTN updates, the data shuffle time is further improved by over $60$\% for all data volumes. 

\begin{figure}[t]
  \centering
  \mbox{
    \subfigure{\includegraphics[scale=0.28]{Figures/testbed_update.pdf}}  
    }
    \mbox{
    \centering
    \small (a) Link utilization before and after the tenant traffic migration.
    }
    %\mbox{
    %\subfigure{\includegraphics[scale=0.63]{data_shuffle.pdf}}  
    %}
	%\mbox{
    %\centering
    %\small (b) Data shuffle time for various data volumes.
    %}    
    \mbox{
    \subfigure{\includegraphics[scale=0.63]{Figures/testbed_updates_new.pdf}}  
    }
    \mbox{
    \centering
    \small (b) Link utilization of three routing candidates over time. 
    }
  \caption{Testbed experiments for fulfilling bandwidth requirement for a tenant (running MapReduce jobs) through
  tenant traffic migration.
  The tenant traffic migration performed at $60$s introduces zero loss. The new tenant is embedded at $100$s.
  }
  \label{fig:bandwidth}
\end{figure}
\normalsize


\noindent\textbf{Shuffle speed up:} 
To demonstrate \sys's benefits for fulfilling bandwidth requirements, we 
create a new tenant to perform data shuffle on our testbed. 
We adopt the same network topology and background link utilization used in the 
testbed experiments in \S \ref{sec:FCT}.  
The new tenant's $10$ VMs are evenly spanning
across $\texttt{H}_\texttt{1}$ and $\texttt{H}_\texttt{3}$. 
The tenant's application performs a $5$-to-$5$ data shuffle between VMs 
located in different hypervisors. 

To embed the new tenant, \sys has $3$ routing 
candidates based on the topology: 
$\texttt{E}_\texttt{1}\texttt{-C}_\texttt{1}\texttt{-E}_\texttt{2}$, $\texttt{E}_\texttt{1}\texttt{-C}_\texttt{2}\texttt{-E}_\texttt{2}$ and $\texttt{E}_\texttt{1}\texttt{-C}_\texttt{3}\texttt{-E}_\texttt{2}$. Then 
it can explicitly embed the VTN  
into $\texttt{E}_\texttt{1}\texttt{-C}_\texttt{1}\texttt{-E}_\texttt{2}$, 
which has the largest available bandwidth among all candidates 
(Figure \ref{fig:bandwidth}(a)). Furthermore, we can adjust the 
existing VTNs by shifting the traffic from core 
switch $\texttt{C}_\texttt{1}$ to $\texttt{C}_\texttt{2}$, who has enough capacity to 
hold the new traffic. Thus the MapReduce data shuffles can be further
accelerated via the newly updated $\texttt{E}_\texttt{1}\texttt{-C}_\texttt{1}\texttt{-E}_\texttt{2}$, as illustrated in 
Figure \ref{fig:bandwidth}(b).
Note that we are only re-allocating network resources instead of performing VM
migration in our experiments. 
%which can be expensive~\cite{vm_migration}. 
%we cannot shift all traffic so that 
%$\texttt{E}_\texttt{1}\texttt{-C}_\texttt{1}\texttt{-E}_\texttt{2}$ has 
%almost zero utilization. This is because the background tenants whose 
%VMs are placed in $\texttt{H}_\texttt{1}$ and $\texttt{H}_\texttt{3}$ 
%need to consume the bandwidth as well. 
%As illustrated in Figure \ref{fig:bandwidth}(b), 
%with the management flexibility offered by \sys, the data shuffle time for can be further
%reduced by ${\sim}60$\% after tenant traffic migration.

\noindent\textbf{VTN updates:} Figure \ref{fig:bandwidth}(b) shows the physical 
path utilization over time. The background VTN updates are performed at time $60$s. 
It is clear that the updates introduce zero traffic loss. This is because the 
network operators are aware of the physical links used by each tenant. 
Thus they can re-configure VTNs for the background tenants to smoothly 
migrate their traffic to new paths that have enough capacity to hold the traffic. 
Thus the updated tenants experience no losses. At time $100s$, we embed the 
new VTN.  
%to the network $\texttt{E}_\texttt{1}\texttt{-C}_\texttt{1}\texttt{-E}_\texttt{2}$. 


\noindent\textbf{Bandwidth guarantees:} 
In cloud computing, bandwidth guarantee is 
proposed to provide performance predictability in the shared 
environments~\cite{predictable,secondnet}. In multi-tenant data centers, 
bandwidth guarantee embedding allows network operators to assign 
desired bandwidth for tenants' virtual links. 

With the help of \sys, network operators can easily enforce the virtual link 
bandwidth guarantees. Specifically, since \sys first outputs 
all desired routing candidates, network operators can explicitly 
choose one of them which has enough capacity to satisfy the bandwidth 
requirement. If none of the candidates can meet the requirement, network operators 
can perform background VTN updates so as to create enough space to satisfy the tenant's requirement. 
Furthermore, when the current embedding can no longer satisfy the requirement due to network dynamics, 
\sys can configure new network to satisfy the requirement or even perform 
VM migration if necessary. Although \sys does not 
create new techniques for performing VM migration or propose new bandwidth allocation algorithm, 
its explicit tenant routing control significantly reduces the management efforts for performing these tasks 
since network operators are aware of what network resource is used by each tenant. 

\fi


\iffalse
\subsection{Accelerating Data Transferring}
To avoid performance degradation due
to competing traffic with other tenants, network operators often consider
congestion before embedding VTNs, i.e., congestion-aware embedding.
Congestion-aware embedding helps reduce both the data center holistic congestion experienced by
all tenant networks and specifically individual virtual links~\cite{pfabric, deadline, pdq}. 

As mentioned, the choice of the objective function is open to the network
operator. To have a simplified objective function without losing
generality, we estimate the average congestion level of the virtual links in the VTN
to score the routing candidates. The congestion level of a virtual link
is estimated as the congestion level of the highest utilized physical link
embedding the virtual link, while the congestion level of a physical link is
estimated by the number of virtual links that the physical link hosts. 

%For a tenant with $k$ virtual links, \sys produces $m$ virtual
%network candidates $\{T_1,...,T_m\}$. For each candidate, we known
%aware of the exact mapping between virtual links and physical links so that they
%can learn the congestion experienced by each virtual link. Thus the objective
%function to determine the least congested candidate is $g =
%\min_{\{T_1,...,T_m\}} \frac{1}{k}\sum c(l_i, T_j)$, where $c(l_i, T_j)$ is the
%congestion extent measured for virtual link $l_i$ if candidate $T_j$ is elected.
%Since one virtual link may associate with multiple physical links (\eg in part
%(d) of Figure \ref{fig:mst}, the virtual link between VM1 and VM2 is carried by
%$3$ physical links), the congestion extent for each virtual link is measured by
%the \emph{highest} utilization of all the associated physical links since that
%link is expected to be the bottleneck.

\comment{add more experiments details}
Then we compare the average congestion experienced by
the virtual links when one of two VTNs is selected. Specifically, we develop a
client and server program for each virtual link to generate traffic. The source
(client) of each virtual link samples one flow size from one of the two
realistic data center workload distributions (Figure \ref{fig:flow}) and starts
transmitting to the destination (server). The two workloads are based on
empirically observed traffic patterns in deployed data centers. The first one
(Figure \ref{fig:flow:a}) represents a large enterprise  data center
workload~\cite{conga} and the second one (Figure \ref{fig:flow:b}) is from a
large cluster providing cloud services~\cite{vl2}. Both distributions are
heavy-tailed since a small fraction of flows contribute most of the bytes.
Similar to previous work~\cite{why_fct, conga, pfabric}, we use the Flow
Completion Time (FCT) as the major metric to quantify the congestion.


\begin{figure}[t]
  \centering
  \mbox{
    \subfigure[\label{fig:flow:a}Enterprise workloads.]{\includegraphics[scale=0.38]{Figures/flow_dis1.pdf}}  
    \subfigure[\label{fig:flow:b}Cloud cluster workloads.]{\includegraphics[scale=0.38]{Figures/flow_dis2.pdf}} 
    }
  \caption{Realistic data center workloads. \comment{add flow-size filter}}
  \label{fig:flow}
\end{figure}


In order to compare different routing options, we compute the flow completion
time for large data transferring flows, expecting that a better routing option
will end with a shorter flow completion time. 

\begin{figure}[t]
  \centering
%    \subfigure[Enterprise workloads.\label{fig:testbed_cong_aware:a}]{\includegraphics[scale=0.6]{testbed_congestion_aware_embed.pdf}}
   % \subfigure[Cloud cluster workloads.
    \label{fig:testbed_cong_aware:a}]{\includegraphics[scale=0.6]{Figures/testbed_congestion_aware_embed_cdf2.pdf}}
  \caption{Normalized acceleration for data flows. \sys can shorten flow
  completion time significantly. \comment{Trial number to Trial NO.}}
  \label{fig:testbed_cong_aware}
\end{figure}


\para{Small-scale real testbed results.}
%Besides evaluating the acceleration for large flow completion time in
%simulation, 
In one trial, we create a new tenant whose $10$ VMs are evenly assigned between
hypervisors $\texttt{H}_\texttt{1}$ and $\texttt{H}_\texttt{3}$ in OpenStack
environment. In total, we perform $40$ trials and after each trial, every
virtual link transmits $10$ random large-size flow streams picked up from
Figure~\ref{fig:flow}. 
For each new VTN, to compare the routing chosen by \sys with the ones
selected by other three solutions, i.e., ECMP, the bottomline, and the local, 
we normalize the flow completion time of \sys offered routing based on the one of the
``bottomline'' solution offered. Figure~\ref{fig:testbed_cong_aware} shows the
normalized flow completion time as function of the attempt trial NO. As we can
see that in most cases, \sys can reduce the flow completion time by 20\%-40\%.
Due to space limitation, we omit the results of ECMP and the local solution in
Figure~\ref{fig:testbed_cong_aware}. The difference between ECMP and the bottomline in our experiments is small
because we use random hash function to hash flow headers and tenant IDs
respectively. \comment{results for local}.

\comment{move this to conclusion} Consequently, the tenant hashing may result in overwhelming some already congested links and switches, which in turn causes degrading performance. In some trials, \sys has a ${\sim}1.7\times$ reduced FCT compared with T-ECMP and on average \sys outperforms T-ECMP by ${\sim}20$\%. The results for the two data center workloads are similar. 

\fi

\iffalse
\subsection{Efficient Tenant Management}
In this section, we show that the \sys helps the network operators easily manage the tenant networks. Data center fabric is often constructed with redundant physical links to spread the traffic load (\eg using ECMP). Thus, without explicit in-network tenant routing control, one tenant's traffic may span cross large numbers of physical links and switches although it only consumes a tiny fraction of the total computation resources. Figure \ref{fig:manage} shows the number of physical links used by each tenant when we perform flow-level ECMP. As we can see from the results, without explicit tenant routing control, one tenant's traffic may span cross up to $6\times$ more physical links compared with \sys.

\begin{figure}[t]
  \centering
  \mbox{
    \subfigure{\includegraphics[scale=0.62]{Figures/ecmp_opreduce_3load.pdf}}
  }
  \caption{The number of physical links used by each tenant without explicit routing control.}
  \label{fig:manage}
\end{figure}



The poor tenant traffic isolation increases the difficulty of tenant management. For instance, it is hard to perform monitoring, measurement and trouble shooting for a specific tenant since it is difficult to locate its traffic. Furthermore, when ``hot spots" appear in the data center, network operators cannot effectively ``cool down'' the congested links by detouring the traffic to other available paths because they are not aware of which tenants contribute to the hot spots. Similarly, in case of link failures, network operators cannot determine the affected tenants to re-route their traffic in time. \sys is a scalable and efficient system framework that allows network operators to perform explicit tenant-level routing control, which in turn enables efficient tenant management. 
\fi

\subsection{System Properties}\label{sec:system_evaluation}
%In previous sections \S\ref{sec:FCT} and \S\ref{sec:bandwidth}, we
%have evaluated the performance benefits offered by \sys. 
%In this section, we examine  \sys's system properties.
%using our real testbed 
%to confirm that \sys does meet the requirements for common practices. 
%In this section, we present system evaluation.

\subsubsection{Search Cost Reduction}\label{sec:search_cost_reduction}
%In multi-tenant datacenters, tenant routing updates are all-time tasks. 
The number of routing update requests is affected by the amount of embedded 
tenants, \ie the load degree. Figure~\ref{fig:seach_cost_reduction} plots search 
cost reduction under various loads for $k{=}16$ fat-tree topology. 
Although the absolute number of routing updates increase 
as load degree increases, the normalized search cost actually reduces. 
This is because \sys's knowledge base about routing candidates for 
various VM locations also expands as the load degree increases. 
As a result, the cache hit ratio dramatically increases as well (Figure~\ref{fig:catch_hit_ratio}). 
Thus, in spite of the numerous routing updates, \sys introduces small topology search cost. 

\begin{figure}[t]
	\centering
	\mbox{
		\subfigure[\label{fig:seach_cost_reduction} Search cost reduction]{\includegraphics[scale=0.23]{Figures/search_cost_reduction.pdf}}
		\subfigure[\label{fig:catch_hit_ratio} Cache hit ratio]{\includegraphics[scale=0.23]{Figures/cache_hit_ratio.pdf}}
	}
	\caption{In spite of the numerous routing updates as load degree increases, 
		\sys introduces small search cost since the cache hit ratio increases dramatically.  
	}
	\label{fig:search_cost}
\end{figure}

\subsubsection{Routing Cache Size}\label{sec:evaluation:cache_size}
%\sys's decoupled search and embedding design allows routing candidates to be reused. 
%We investigate the cache size in different settings. 
%How we implement routing cache is described in \S\ref{sec:implementation}. 
%The cache size is decided by two factors: the topology and the distribution of VM placement. 
The routing cache size is affected by two factors: the topology and the average VTN scale.  
The topology affects the cache size because it affects the number of routing candidates 
for one VM placement. The VTN scale affects the cache size since it determines 
the number of physical links in one routing candidate. 
%The topology affects the cache size because the physical links
%carrying VTNs' virtual links vary. 
%In a multi-tenant data center, network
%operators often attempt to place VMs in the same VTN locally to reduce the
%distance between VMs, making the number hypervisors hosting VMs tend to be
%small. If most of the VTNs are hosted by smaller number of hypervisors, the
%diversity of routing will be less accordingly. Thus, the expected number of
%hypervisors hosting a VTN is another critical factor determining the cache size. 

Figure~\ref{fig:cache_size_diff_VTN} plots cache sizes with respect to the number of 
tenants and the average VTN scales in $k{=}16$ fat-tree topology. 
The cache size increases with the average VTN scale and linearly grows with the number of tenants. 
However, even with very sporadically distributed VTNs, \ie large average VTN scales, 
caching routing candidates for $10$K tenants consumes no more than $40$MB memory. 
Even if we consider a much larger $k{=}32$ fat-tree datacenter with over 
$8$K servers, the cache size for $10$K tenants is about hundreds of Megabytes 
(Figure~\ref{fig:cache_size_diff_topo}), 
which can be easily managed by commodity servers with gigabytes of memory. 

\begin{figure}[t]
	\centering
	\mbox{
		\subfigure[\label{fig:cache_size_diff_VTN} Various VTN scales]{\includegraphics[scale=0.23]{Figures/cache_size_16K.pdf}}
		\subfigure[\label{fig:cache_size_diff_topo} Various topologies]{\includegraphics[scale=0.235]{Figures/cache_size_diff_topo.pdf}}
	}
	\caption{The routing cache size under various settings.}
	\label{fig:cache_size}
\end{figure}


\subsubsection{Switch Configuration Latency}\label{sec:evaluation:switch_config}
Both SDN switches and legacy switches may co-exist in today's datacenters~\cite{hybnet}. 
Configurations on OpenFlow Switches can be finished almost 
in real time via SDN controllers such as OpenDayLight~\cite{opendaylight}, but it takes 
non-trivial time to configure legacy switches. 
Thus, to ensure that routing enforcement does not become 
the bottleneck for routing update, \sys designs a network 
action container to properly aggregate configuration tasks so as 
to reduce the overall configuration delay.  


In \sys's prototype, one switch configuration task is about associating one VLAN tag on 
a certain port of a switch. We notice that configuring a single port on a legacy switch 
takes almost the same amount of time as configuring multiple ports on the switch. 
Thus, our network action container aggregates all 
configuration tasks on the same switch together to perform batch configuration so as 
to reduce the overall configuration delay. Meanwhile, 
batch configurations for different switches are executed simultaneously via multi-threading. 
Figure~\ref{fig:config_delay} plots the measured configuration delay on our testbed. 
The results show that even if we simultaneously configure $24$ ports on 
one switch and on each port we configure $24$ 
VLAN tags ($576$ single configuration tasks), the overall configuration time is less than $1.5$ times the 
delay for configuring just one VLAN tag on a single port. 
%Without the network action container, the configuration time would be linear to the number
%of ports and the number of VLAN tags to be configured on each port, which could be up to hundreds of seconds. 
Thus, with the network action container, routing enforcement can be finished timely
so that it will not be a bottleneck in practice. 

\begin{figure}[t]
	\centering
	\mbox{
		\subfigure{\includegraphics[scale=0.53]{Figures/config_time.pdf}}
	}
	\caption{Delay measurements for configuring legacy switches. 
		The dash line indicates the configuration time without using 
		the network action container.
	}
	\label{fig:config_delay}
\end{figure}



\iffalse
\noindent\textbf{Switch configuration delay:}
Both SDN switches and legacy switches may co-exist in today's data
centers~\cite{hybnet}. Configurations on OpenFlow Switches can be finished in real
time via SDN controllers such as OpenDayLight~\cite{opendaylight}, but it takes 
non-trivial time for legacy switches. 
Thus, in order to make sure that VTN embeddings do not become 
the bottleneck for tenant routing management, we develop a network 
action container for \sys to properly aggregate configuration tasks so as 
to reduce the overall configuration delay.  

%Thus, we investigate the overhead for configuring switches to embed a VTN 
%to confirm that \sys is not the bottleneck in updating VTNs. 

In our implementation, one switch configuration task is about associating one VLAN tag on 
a certain port of a switch. We notice that 
configuring one port on one legacy switch and configuring multiple ports on one legacy switch take 
almost the same amount of time. Thus, our network action container aggregates all 
configuration tasks on one switch as a batch and executes the batch simultaneously rather than 
performing configuration task on by one. Figure~\ref{fig:config_delay} shows 
the configuration delay study on our testbed. In fact, even if we simultaneously configure $24$ ports on 
one switch and on each port we configure $24$ 
VLAN tags ($576$ single configuration tasks), the overall delay is less than $1.5\times$ the 
delay for configuring just one VLAN tag on a single port. 
Without the container, the delay will be linear to the number
of ports and the number of VLANs to be configured on each port, which can be up to hundreds of seconds. 
Therefore, with the network action container, configurations for VTN embeddings can be timely
processed as a batch so that overall configuration delay will not become bottleneck in practice. 


%we use VLAN tags to identify VTNs. Based on the network
%action container in our system (\S\ref{sec:implementation}), 
%the configuration operation on a switch consists of 
%a list of ports and VLANs to be associated with each port. 
%Thus, the configuration
%delay is decided by the number of VLANs and the number of ports.
%In our experiments, we control the number of ports and the number of VLANs to tag on each port 
%to learn the configuration delay. 
%Meanwhile, we run end-to-end \texttt{ping} to test reachability,
%and count the delay based on the first arrival probe on the destination end. 

%For legacy switches, according to Figure~\ref{fig:config_delay}, neither the number of ports nor the
%number VLANs affects the configuration delay much. 
%Even if we increase the
%number of ports to configure up to 24, the configuration delay is just XXX times
%the one that the number of ports is merely 1. 
%In fact, even if we configure $24$ ports and on each port we configure $24$ 
%VLAN tags ($576$ single configurations), the overall delay is less than $1.5\times$ the 
%delay for configuring just one VLAN on a single port. 
%The marginal overhead of
%configuration delay is offered by proper aggregation of configurations at the network
%action container. Without the container, the delay will be linear to the number
%of ports and VLANs to be configured on each port, which can be up to hundreds of seconds. 
%The configuration delay for OpenFlow switches
%is negligible, \ie always less than 1s. 


\begin{figure}[t]
	\centering
	\mbox{
		\subfigure{\includegraphics[scale=0.53]{Figures/config_time.pdf}}
	}
	\caption{Delay measurements for configuring legacy switches. Each solid curve represents for a
		given number (1, 8, 24) of ports to configure,  the
		configuration delay as a function of the number of VLANs to be configured on each port. 
		The dash line indicates the delay w/o the network action container.
	}
\end{figure}


\begin{figure}[h]
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[scale=0.35]{Figures/cache_size_16K.pdf}
\caption{Cache size w.r.t. average VTN scales and \# of tenants.}
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[scale=0.35]{Figures/cache_ratio.pdf}
\caption{Hit ratio w.r.t. \# of previously received VTN requests.}\label{fig:hit_ratio}
\end{minipage}
\end{figure}




\noindent\textbf{Routing cache size:}
%\sys's decoupled search and embedding design allows routing candidates to be reused. 
%We investigate the cache size in different settings. 
%How we implement routing cache is described in \S\ref{sec:implementation}. 
%The cache size is decided by two factors: the topology and the distribution of VM placement. 
The routing cache size is decided by two factors: the topology and the average VTN scale.  
The topology affects the cache size because it affects the number of routing candidates 
for one VM placement. 
The VTN scale affects how many physical links one routing candidate has. 
%The topology affects the cache size because the physical links
%carrying VTNs' virtual links vary. 
%In a multi-tenant data center, network
%operators often attempt to place VMs in the same VTN locally to reduce the
%distance between VMs, making the number hypervisors hosting VMs tend to be
%small. If most of the VTNs are hosted by smaller number of hypervisors, the
%diversity of routing will be less accordingly. Thus, the expected number of
%hypervisors hosting a VTN is another critical factor determining the cache size. 

Figure \ref{fig:cache_size} shows the cache sizes with respect to the number of 
tenants and the average VTN scales in $k{=}16$ fat-tree topology. 
The cache size increases with the average VTN scale and glows linearly with the number of tenants. 
However, even with very sporadically distributed VTNs, \ie large average VTN scales, 
caching routing candidates for $10$K tenants consumes no more than $40$MB memory. 
Even if we consider a much larger $k{=}32$ fat-tree data center, which has over 
$8$K servers, the cache size for 
$10$K tenants is about hundreds of Megabytes (not plotted due to space limit), 
which can be easily managed by PCs with gigabytes of memory. 
Therefore, caching the search results for future use cannot become a bottleneck in practice. 


We first fix the topology to a $k{=}16$ fat-tree topology to investigate the
impact of VTN scale. We carry out $4$ experiments, in each of
which we randomly generate VTNs but fix the VTN scale to $2$, $3$, $4$
and $5$, respectively. As we can see from the result 
(Figure~\ref{fig:cache_size}), 
when the data center hosts $10$K tenants, the cache 
size is around $40$MB, which can be easily managed by PCs with gigabytes of memory. 

Then we investigate how the cache size is affected by the topology. 
Although as the topology size grows the number of alternative routing candidates may
increase significantly, the cache size is still capped by 
the expected number of hypervisors host a VTN. 
Due to space limitation, we omit the figure here. The results show that even in
$k=32$ fat-tree data center, which has over $8$K servers, the cache size for
hosting $10$K tenants is less than $100$MB, and the cache size is still linearly
proportional to the number of tenants. Therefore, caching the routing 
search results for future use can never be a bottleneck in the implementation. 


\noindent\textbf{Cache hit ratio:} We close our system evaluation by showing 
the hit ratio for the routing cache, \ie given a new VTN embedding request, what is the probability 
that we can reuse the cache results. 
We use the $k{=}16$ fat-tree topology and set the average VTN scale to $4$. 
Network operators may tend to allocate VMs for one tenant within one pod so as to reduce 
the average hops of VM communications. 
Figure \ref{fig:hit_ratio} shows that as the number of
previously received VTN embedding requests grows, the chance to reuse search results increases significantly.
This is because \sys has more cache results after receiving more embedding requests. 
Note that Figure \ref{fig:hit_ratio} only considers the hit ratio of embedding requests for new tenants. 
For the VTN embedding requests triggered by the routing updates for existing tenants, the 
hit ratio is $100\%$. Therefore, \sys's decoupled design is long-term cost-efficient. 

%We present the routing cache size for different data center topologies hosting varying numbers of tenants in Figure \ref{fig:cache}. Note that the size is calculated for the worst case (all the hypervisors for one tenant are located in different pods). 

%Figure \ref{fig:cache:b} shows the cache sizes for $k=16$ fat-tree topology. We vary the number of hypervisors occupied by each tenant from $2$ to $5$. Figure \ref{fig:cache:b} scales up the topology size. Note that the Clos topology has the same number of servers as $k=32$ fat-tree topology but with oversubscription ratio $2:1$. 

%The results show that even in $k=32$ fat-tree data center, which has over $8$K servers, the cache size for hosting $10$K tenants is less than $100$MB. Therefore, caching the routing search results for future use can never be a bottleneck in the implementation. 

%Let's quantify the cache size for a very large data center fabric. Assume the data center fabric is a $16$-pod fat-tree hosting $10$K tenants. Then the worst case cache size ( is around $5H$ MB, where $H$ is the number of hypervisors occupied by each tenant. As analysed in \S \ref{sec:vm_place}, $H$ is often no more than $5$. Thus the total cache size is around $25$MB, which can be easily managed by commodity servers with gigabytes of memory. 


%In this experiment settings for the congestion aware embedding, the network operators try to find a desired virtual network for each tenant to optimize the FCT performance for certain virtual links which carry latency sensitive flows. In such case, 
\fi

==> Managing Recurrent Virtual Network Updates in Multi-Tenant Datacenters A System Perspective/implementation.tex <==
\section{Implementation}\label{sec:implementation}
%We implement \sys on an OpenStack testbed with networking configured as Figure~\ref{fig:system_arch},
%consisting of a network information database, a network controller (managing in
%both OpenFlow and \texttt{netconf} protocols), and \sys as
%an application of the network controller. Further, \sys includes four major
%modules, \ie the routing search engine, routing cache, the objective functions and a network actions container.

We have a full implementation of \sys. We use OpenStack to create VMs on hypervisors and assign VMs to 
tenants. On our testbed dedicated for experiments, the OpenStack environment 
has $4$ compute nodes as hypervisors that can host about one hundred VMs, 
one network node, and one controller node. Because OpenStack is limited to computation 
virtualization, we unify it with our physical network via an 
OpenDayLight~\cite{opendaylight} controller that uses OpenFlow and \textsf{netconf}~\cite{netconf}
protocols to manage OpenFlow and legacy switches, respectively. 


On our testbed, we allocate a dedicate VLAN tag for each
VTN. Then embedding a VTN is about configuring relevant switch interfaces
with corresponding VLAN tags to achieve reachability. Certainly there could be other 
network virtualization solutions, \eg slices in sliceable
switch~\cite{trema}, VLAN tag stacking~\cite{stacked_vlan}. \sys's 
network controller is extendible to support these virtualization solutions. 
We are aware that VLAN tags are limited to $4096$ values 
which may be insufficient in large scale datacenters. To resolve this scalability issue, 
\sys implements a helper component, based on Panopticon~\cite{panopticon}, 
to achieve VLAN tag reuse in hybrid datacenters with both legacy and OpenFlow switches. 

%We implement \sys on our testbed as illustrated in Figure~\ref{fig:system_arch},
%consisting of a network information database, a network controller, \sys's
%VTN embedding module and the underlay physical data center. 

%We organize our switches into a layered network topology illustrated in Figure \ref{fig:testbed}. The small scale data center consists of five switches (Core2 and Core3 are OpenFlow switches and the rest are Juniper switches) and four racks of physical servers which are able to host hundreds of virtual servers. Three core switches are inter-connecting two pods. Each server connects to one edge switch with one uplink and each edge switch is connecting all three core switches with three uplinks.
%\sys makes optimal decisions merely based on the information it gets from the network information database, and thus \sys cannot tell it is a simulated testbed or real physical testbed, which means that the system evaluation of \sys is not affected by whether the network information database's data is simulated or real. In our experiments, the network information database is feed with either information collected from a small real testbed or emulated network states using realistic traffic load.

% Probably we can take a photo of our switches

\iffalse
\begin{figure}[h]
  \centering
  \mbox{
    \subfigure[Network topology.]{\includegraphics[scale=0.3]{Figures/testbed.pdf}}  
    \subfigure[Embedding examples.]{\includegraphics[scale=0.3]{Figures/testbed_embed.pdf}} 
    }
  \caption{\footnotesize Part(a) is the network topology in our implementation. Part (b) illustrates the embedding examples for two tenants. The first tenant is allocated VMs in rack 2 and rack 3 whereas the second tenant spans cross rack 1 and rack 4.}
  \label{fig:testbed}
\end{figure}
\normalsize


%\subsection{OpenStack}
We utilize OpenStack to create VMs on hypervisors and assign VMs to 
tenants. Our OpenStack environment has $4$ compute nodes as hypervisors 
which can host fewer than one hundred VMs, one
network node, and one controller node. 
Because OpenStack is limited to computation virtualization and endhost configuration, we
unify it with our physical network via an OpenDayLight~\cite{opendaylight} controller 
which uses both OpenFlow and \texttt{netconf}
protocols to manage OpenFlow switches and legacy switches, respectively, on our testbed. 
 

To enforce in-network routing control, network operators need to guide switches how to 
forward packets for a certain tenant. 
In our prototype implementation, we allocate a dedicate VLAN tag for each
VTN and install forwarding rules on switches based on the VLAN tag. 
We realize that VLAN tag space is limited to $4096$ values which may be insufficient 
for large scale data centers. To resolve the scalability issue, we can adopt the Panopticon~\cite{panopticon} which 
allows VLAN tag reuse in hybrid data centers with both legacy and OpenFlow
switches. As more and more data centers are built with full OpenFlow switch 
deployment, network operators will have larger space to install more flexible forwarding rules~\cite{infinite} 
to enforce in-network routing control. 

%\subsection{Network Virtualization}\label{sec:net_virtual}



%In our testbed, we allocate a dedicate VLAN tag for each
%VTN, then embedding a VTN is about configuring the relevant switch interfaces
%with the corresponding VLAN tag to achieve reachability. Certainly there could be
%network virtualization solutions other than VLANs, \eg slices in sliceable
%switch~\cite{trema}, VLAN tag stacking~\cite{stacked_vlan}. But which solution to use
%is up to the implementation of the network controller (\eg OpenDayLight, Trema~\cite{trema}), and is independent from \sys.     

%To speed up virtual network configurations in our testbed, we append
%a network actions container to the end of \sys to properly aggregate the VLAN configuration tasks. 
%Each switch is allocated a configuration task queue to buffer 
%VLAN tasks. As the configurations in a same queue are applied to the same
%switch, these configurations can be issued to the switch at the same time
%instead of one by one in sequence.
%Thus, when a new request arrives (could be caused by either new tenant requests or 
%updates from existing tenants), it will iterate over switches' task queues and 
%check if any configuration can be folded into the pending tasks. Note that since configurations on different
%switches are processed independently and can be parallelized, the overall
%configuration delay will not 
%inflate as the number of switches increases (as discussed in \S\ref{sec:benchmark}). 

\comment{move this to evaluation}
C on OpenFlow Switches can be finished real
time via OpenDayLight. However, it takes dozens of seconds to perform a single
configuration for one tenant on one port on Juniper switches. Fortunately, the
configurations for multiple tenants on multiple ports at the same switch can be
processed as a batch and the overall configuration time does not linearly
increase with respect to the number of single configuration. In fact, as
illustrated in Figure \ref{fig:config_delay}, the increase of overall
configuration time is marginal. In the extreme scenario of our evaluation where
we configure $24$ tenants on all the $24$ ports of a switch (totally it will be
$24*24=576$ single configurations), the configurations can be finished within
$25$ seconds. The configurations on different switches can be processed
in parallel.


Therefore, the configuration delay is still acceptable in hybrid (containing both legacy and
OpenFlow switches~\cite{hybnet}) or even legacy data centers. In our testbed, we
need to configure two ports on each switch for one VTN. The configuration delay
is illustrated by the dash line in Figure \ref{fig:config_delay}).

\begin{figure}[t]
  \centering
  \mbox{
    \subfigure{\includegraphics[scale=0.6]{Figures/config_time.pdf}}
    }
  \caption{Configuration delay study for Juniper switches. The dashed line represents the delay for embedding VTNs in our testbed.}
  \label{fig:config_delay}
\end{figure}

\begin{figure}[t]
  \centering
  \mbox{
    \subfigure[\label{fig:cache_a} Diff. \# of hypervisors.]{\includegraphics[scale=0.42]{Figures/cache_size_16K.pdf}}
    \subfigure[\label{fig:cache:b} Diff. topologies.]{\includegraphics[scale=0.42]{Figures/cache_size_diff_topo.pdf}}
    }
  \caption{Cache size evaluation. We use $k=16$ fat-tree topology in Part(a) and vary the number of hypervisors one tenant occupies from $2$ to $5$. Part(b) shows the cache sizes for different topologies with fixed hypervisors ($3$) per tenant.} 
  \label{fig:cache}
\end{figure}
\fi

% not necessary since the informance is on PC not on router or switches which has very small amount of memory
%\subsection{Cache for Topology Search}\label{sec:topo_search}
%\comment{do not use vague terms like VTN candidates}
%The search results for routing candidates are cached using a hash data
%structure, where the key is the hash of the VM placement in terms of a list of
%hosting hypervisors, and the value is a list of routing candidates. Each
%candidate is stored as a list of physical link IDs, which can be used to retrieve 
%link related information (\ie utilization) from the network information database. 
%In \sys's implementation, we allocate $32$ bits for both the hash key and physical link IDs. 

%In \S \ref{sec:benchmark}, we show that even in large scale $k{=}32$ fat-tree data center, 
%which has over $8$K servers, the cache size for hosting $10$K tenants is 
%around hundreds of Megabytes, which can be easily managed by PCs with gigabytes of memory.
%Therefore, caching the routing search results can never be a bottleneck in 
%the implementation. 

%We present the cache size for different data center topologies hosting varying numbers of tenants in Figure \ref{fig:cache}. Note that the size is calculated for the worst case (all the hypervisors for one tenant are located in different pods).

%Figure \ref{fig:cache:b} shows the cache sizes for $k=16$ fat-tree topology. We vary the number of hypervisors occupied by each tenant from $2$ to $5$. As we can see from the result, for the $k=16$ fat-tree data center hosting $10$K tenants, the cache size is around $40$MB, which can be easily managed by PCs with gigabytes of memory. Figure \ref{fig:cache:b} scales up the topology size. Note that the Clos topology has the same number of servers as $k=32$ fat-tree topology but with oversubscription ratio $2:1$. The results show that even in $k=32$ fat-tree data center, which has over $8$K servers, the cache size for hosting $10$K tenants is less than $100$MB. Therefore, caching the search results for future use can never be a bottleneck in the implementation. 

%Let's quantify the cache size for a very large data center fabric. Assume the data center fabric is a $16$-pod fat-tree hosting $10$K tenants. Then the worst case cache size ( is around $5H$ MB, where $H$ is the number of hypervisors occupied by each tenant. As analysed in \S \ref{sec:vm_place}, $H$ is often no more than $5$. Thus the total cache size is around $25$MB, which can be easily managed by commodity servers with gigabytes of memory. 


==> Managing Recurrent Virtual Network Updates in Multi-Tenant Datacenters A System Perspective/intro.tex <==
\section{Introduction}
Along with the rise of cloud computing, multi-tenant datacenters grow into the
scale of tens thousands of servers hosting millions of tenant VMs~\cite{amazon_dc_size}.
Managing multi-tenancy at such a scale to ensure efficiency,
scalability and agility is a challenging problem drawing considerable 
research and engineering attention. Prior proposals~\cite{netlord, vmware} place
major management effort at hypervisors for the sake of easy configuration and implementation,
whereas little effort has been made to manage \emph{in-network} routings, 
particularly at the granularity of tenants. As a result, 
although the VM locations of each tenant are decided, datacenter network operators 
lose the visibility of actual in-network traffic forwarding for each tenant. 

The lack of tenant-level traffic accountability and routing control could lead
to various limitations. From the perspective of business, 
network operators cannot customize tenant routings in accord with
tenants' service level agreements (SLA) (\eg latency, bandwidth, reliability or security
requirements), which may close the door for such a business model in the virtual private
cloud (VPC) market. From the perspective of management, 
in case of resolving hot spots in datacenters, for instance, it is difficult 
to determine the affected tenants and effectively re-route 
their traffic around congestion in time. 

Thus, it is desirable to have explicit tenant routing control. 
The traditional way to achieve tenant routing management relies on topology search  
coupled with an objective function to greedily find the desired overlay network 
for each tenant. Although instant network configuration is   
technically enabled by SDN~\cite{openflow}, 
the conventional approach still has at least two shortcomings. 
First, tenant routing updates in our production datacenters are recurrent, which can be triggered 
by various reasons including network load dynamics, tenant arrivals/departures, hot spots, 
link failures and so on. Repeatedly performing topology search for each routing update 
will impose significant search cost. Second, a tenant routing is updated typically to 
fulfill certain goals. However, it is uncertain that topology search coupled with 
an objective function is sufficient to achieve any goal. For instance, optimizing a performance metric depending 
on virtual links (\ie VM pair communications) is subject to sub-optimality since 
the mapping between physical links and virtual links is unknown during topology 
search (\S\ref{sec:embedding_goal}). 


To address these issues, we propose \sys, a novel search and optimization 
\emph{decoupled} design for routing management. For each tenant-routing update, 
\sys first comprehensively searches all desired overlay candidates
considering only the tenant's VM locations. Then it applies 
a global objective function over these candidates to finalize the most desired one. 
\sys's decoupled model offers at least two advantages. 
First, since topology search is not directed by any objective function, 
search results are general and can be reused across routing updates that 
share the same VM locations: \ie regardless of their goals, topology search 
for future routing updates is saved as long as their VM locations have been explored. 
%of the same tenant and other tenants whose 
%VMs are hosted by the same set of hypervisors. 
Second, with the global view of all routing candidates, objective functions 
are not limited to be greedy and local. This eliminates 
the possibility of sub-optimality even when optimizing complex performance metrics, 
for instance, involving virtual links. 

One concern of the decoupled design may be that comprehensively finding 
all desired overlay candidates for a tenant can be expensive. 
However, since the VMs of one tenant are typically
spanning across a few racks, we can reduce the search space to a 
subgraph of the entire topology. Further, most data 
center topologies (\eg VL2~\cite{vl2}, fattree~\cite{fat-tree})
are hierarchically organized into several layers and network traffic 
is never forwarded back and forth between different 
layers. We can adopt these properties to further refine the search space. 
Our proposed algorithm can perform comprehensive 
topology search in polynomial time (\S \ref{sec:search_brief}).


\begin{figure*}[t]
	\centering
	\begin{tabular}{|c|c|c|c|}
		\hline
		\subfigure{\includegraphics[scale=0.2]{Figures/inter-mst.pdf}}&
		\subfigure{\includegraphics[scale=0.2]{Figures/default-mst.pdf}}&
		\subfigure{\includegraphics[scale=0.2]{Figures/alter-mst.pdf}}&
		\subfigure{\includegraphics[scale=0.2]{Figures/optimal-mst.pdf}}\\
		\hline
	\end{tabular}
	\begin{tabularx}{\textwidth}{*4{>{\centering\arraybackslash}X}}
		\small (a) Intermediate. &
		\small (b) Default. &
		\small (c) Alternative. &
		\small (d) Optimal. \\
	\end{tabularx}
	\caption{Due to the lack of mapping between virtual links and physical links, 
		conventional search \& optimization coupled solution is subject to sub-optimality when optimizing 
		performance metrics depending on virtual links.}
	\label{fig:mst}
\end{figure*}

We implement a prototype of \sys and perform extensive evaluations 
to validate its design goals. On the one hand, we show that \sys greatly 
reduces the search cost for tenant-routing updates, meanwhile imposing  
small system overhead for managing large scale datacenters (\eg small 
routing cache size and agile network configuration). On the other hand, 
we demonstrate that \sys is able to achieve complex optimization goals 
for routing updates, yielding significant networking performance gain  
over common practice. 

\iffalse
Along with the rise of cloud computing, multi-tenant data centers grow into the
scale of thousands of switches and servers to host tens of thousands of 
tenant Virtual Machines (VMs)~\cite{amazon_dc_size, amazon_dc_growth}.
Managing multi-tenancy at such a scale to ensure efficiency,
scalability and agility is a challenging problem drawing considerable research
and engineering attention. 
Most solutions~\cite{netlord, vmware} place
management effort at only hypervisors for the sake of easy configuration and implementation,
whereas little effort has been taken to \emph{in-network} routing management, particularly at the
granularity of tenants, \ie 
although network locations of VMs are decided, data center operators 
lose the ability to control the in-network forwarding 
(discussed in \S\ref{sec:background}). 


Lack of the tenant-level traffic accountability and routing control could lead
to various limitations for network operators. From the perspective of business, 
network operators cannot customize routing configurations in accord with
tenants' service level agreements (SLA) (\eg latency, bandwidth, reliability or security
requirements), which may close the door for such a business model in virtual private
cloud (VPC). From the perspective of management, 
in case of resolving congested links in data centers, for instance, it is difficult for
network operators to determine the affected tenants and effectively re-route their traffic around congestion in time. 

In order to accomplish in-network tenant routing management in multi-tenant datacenters, 
network operators need to explicitly find an overlay network in the whole data center for each tenant 
and then ``embed" its network into the overlay. Although instant network configuration is   
technically enabled by software-defined networking (SDN)~\cite{openflow,openflow_spec}, 
we still need to address the following two major challenges before having 
a scalable and efficient solution to achieve tenant routing management in multi-tenant data centers. 
To begin with, 
%tenant routing embeddings happen at all times in multi-tenant data centers.  
frequent arrivals of new tenants and 
routing updates to adapt the existing tenant networks to network dynamics 
could trigger considerable amounts
of tenant network embedding requests. 
%Each request is about searching for a
%suitable overlay network on top of the whole data center network to embed one tenant's network.
As each embedding request involves overlay search, 
such huge amounts of embedding requests can introduce non-trivial topology search cost. 
Furthermore, embedding one tenant network requires more than simply 
finding a random overlay, but finding an overlay that can achieve various 
embedding objectives and requirements proposed by tenants or network operators (\eg 
the bandwidth guarantee embedding proposed in~\cite{secondnet, predictable}). 
However, as embedding objectives become complicated, 
it is uncertain whether these objectives can be achieved merely by the overlay network search. 
For instance, an embedding requirement considering multiple performance metrics (\eg latency, 
bandwidth and reliability) cannot be easily achieved by a 
search algorithm (see more discussion in \S\ref{sec:embedding_goal}).


%As data center networks are augmented by software-defined networking (SDN)~\cite{openflow}, 
%regular instant routing updates are technically enabled using protocols such as OpenFlow~\cite{openflow_spec}. 
%Due to such increased feasibility, various network routing updates oriented by different
%objectives or goals have been proposed, such as short latency, low path
%inflation, large bandwidth, high reliability, and so forth~\cite{alizadeh2012less,b4,swan}.

%Therefore, to enable efficient management, network operators should put more
%emphasis on in-network routing control at the granularity of tenant.
%Specifically, network operators should explicitly configure a routing for each
%tenant (essentially a spanning tree connecting all its VMs) and confine its
%traffic within own virtual network to ensure traffic accountability. Based on
%such design philosophy, network operators need to select routings for tenants,
%regularly update routings to keep high resource utilization efficiency and
%perform routing optimizations to best satisfy tenants' flavours.

%Previously, it was not an easy job to perform these routing configurations for network operators, who had to rely on management protocols such as \texttt{netconf}~\cite{netconf}, which is slow, complicated, and error-prone. Nowadays, augmented by software-defined networking, regularly instant routing updates can be technically enabled using protocols such as OpenFlow in data center networks~\cite{openflow_spec, openflow}. Due to such increased feasibility of network routing updates, the desire of network optimization is significantly encouraged. Various optimization demands oriented by different objective functions have been proposed, such as lowest latency, shortest path, minimal configuration cost, highest bandwidth, and so forth~\cite{alizadeh2012less,b4,hong2013achieving}. 

%Usually processing one optimization request works follows two phases: \first proposing a greedy objective function, \second iteratively search across links and using the objective function to dynamically refine the search space of next forwarding hops. The final remaining route is considered the best when the iteration ends. Prim's and Kruskal's minimum spanning tree algorithms follows this process~\cite{kruskals,prims}. 

%However, there is still one step away from having a scalable and efficient solution to achieve



%Furthermore, to make search process efficient, a local objective function\footnote{Any
%objective function proposed to reduce the space over search iterations is
%considered as a local objective function.} is often applied
%during search to confine search space and accelerate search
%progress. However, this inevitably compromises optimality of the found overlay networks. 
%As illustrated in Figure \ref{fig:mst}, it is uncertain whether a performance goal
%can be fulfilled in an intermediate state of search, regardless of 
%what the local objective function is. 




%\begin{noindlist}
%\item {Searching Cost}. 
%\item {Objective Function}. 
%\item {Alternative Routes}. Offering more routing options reduces the chance of overloading particular links. Searching for only one route gives too much pressure to the effectiveness of objective function, which however is not easy as mentioned above. In multi-tenant data center, any link physical link can carry a lot virtual links for tenant networks. Offering one good option is often less preferred than offering multiple not bad options due to reliability concern.
%\end{noindlist}


%a single in multi-tenant data center, such an ``coupled'' optimization process has a few
%short-comings. First, it offers only one routing decision, e.g., one
%minimum spanning tree, but optimization very often is about multiple alternative
%candidates. Second, only greedy objective functions can be
%applied during searching. Some objective functions taking into account
%all links together cannot be coupled into searching. Third, tenants' virtual
%networks cannot re-use searching results because a previous optimal path may
%not be optimal any more due to network dynamics, or 
%objective functions are different across tenants.

To address these challenges, in this paper we propose \sys, a system for automating  
virtual tenant network embeddings in multi-tenant data centers. \sys resolves those 
challenges by proposing a search and embedding ``decoupled'' model. 
Specifically, for each embedding request, \sys first comprehensively searches a list of desired 
overlay network candidates
merely based on the network topology and tenant's VM placement,  then it applies an objective function
over the routing candidates to finalize the one that can  
satisfy the embedding requirement at most. \sys's decoupled model offers at least three advantages: 


\first Topology search results can be cached and reused across different tenant network embeddings: 
there is no need to repeat the overlay search for a
new tenant with the same VM placement as any existing tenants (\ie their VMs are hosted by the same set of
hypervisors).

\second Search effort is independent from network dynamics and embedding goals: 
there is no need to repeat the overlay search for existing tenants 
when their current networks are affected by network dynamics (\eg link congestion or failures) or 
they want to re-embed their networks to achieve a new embedding goal. 

\third Complete flexibility and capability to fulfill embedding goals:  
network operators are no longer restricted to search algorithms to 
achieve tenant embedding goals. Instead, they can design sophisticated algorithms and objective functions 
to accurately evaluate each routing candidate so as to determine the most desired one. 

%\footnote{We expect that VM placement is often decided first before embedding the virtual network


%We realize that the search cost cannot be
%eliminated easily unless the effort in topology search can be de-duplicated.
%In fact, the topology search across tenants are often duplicate. Thus, 
%we propose a search and optimization ``decoupled'' model to re-use 
%search results across tenant network embeddings. 
%we take advantage of such opportunity of re-using search results across embedding tenant
%networks by proposing a search and optimization ``decoupled'' model. 

%\sys comprehensively searches a list of overlay network candidates
%merely based on network topology and its VM placement\footnote{We expect that VM placement is often decided first 
%before embedding the virtual network (discussed in \S \ref{sec:vm_place})}, 
%\second applies an objective function (proposed
%by either the tenant or operators) over the candidates afterwards, and finalizes
%the best among all candidates. As overlay network candidates are not bound
%with any objective functions, the search results can be cached and re-used as
%long as the topology remains the same, which is true because topology changes
%happen much less frequent than network dynamics. We expect such a ``decoupled''
%model offers at least three advantages: 

%\begin{noindlist}
%\item There is no need to repeat the virtual overlay network search for a
%new tenant with the same VM placement as any existing ones (\ie their VMs are hosted by the same set of
%hypervisors).

%\item Search effort is independent from network dynamics. Although it is
%one-time expensive because the search space is not restricted by any local
%objective function, it's long-term cost-efficient.

%\item Since objective functions are applied after search, network
%operators can design sophisticated and global objective functions to
%explicitly fulfill their optimization goals. Thus optimality will not be compromised. 
%\end{noindlist}

One concern of the decoupled design may be that finding all desired overlay 
candidates for a tenant 
%without search space restricted by a specific search objective functions 
can be expensive. 
However, since the VMs of one tenant are typically
spanning across a few racks, we can reduce the search space to a small
subgraph of the entire network so as to confine the search cost.
Further, most data center topologies (\eg VL2~\cite{vl2}, fat-tree~\cite{fat-tree})
are hierarchically organized into several layers and their traffic 
is never forwarded back and forth between different 
layers. We can adopt these properties to further refine the search space. As
presented in \S\ref{sec:search_brief}, our proposed routing search algorithm introduces small
complexity.

In summary, our major contributions are as follows.

\begin{noindlist}
\item We present the design, implementation and evaluation of \sys, a scalable system
for automating virtual tenant network embeddings in multi-tenant data centers. 
%\sys meets the management requirements in multi-tenant data centers (\eg
%traffic accountability and customized routing selection) by operating
%optimization at the granularity of tenant.  
From the perspective of networking management, 
\sys enables effective and agile tenant management (\eg traffic accountability and 
customized routing selection) via explicit tenant-level 
in-network routing control. From the perspective of networking performance, \sys's novel search and embedding 
decoupled design allows network operators to effectively 
achieve various tenant network embedding goals so as to improve a wide range of networking performance. 
%At its design, the search and embedding decoupled design ensures \sys to be scalable to 
%manage large scale multi-tenant data centers. 

%The decoupled search and optimization model of \sys allows network operators to
%apply various objective functions to optimize per-tenant routings as well as achieve
%efficient tenant management. 
%better resource utilization for the whole data center.

\item Via extensive evaluation, we demonstrate that \sys can provide significant networking performance improvement
%We extensively evaluate \sys's networking performance 
for representative tenant embeddings (discussed in \S\ref{sec:evaluation}). 
%We show that \sys can provide significant performance improvement. 
For instance, via better resource allocation among tenants, \sys achieves high 
resource utilization efficiency, which offers up to $5\times$ 
better flow completion time for tenant traffic compared with the common practice. 
%Further, 
%\sys's explicit tenant routing management allows network operators to effectively fulfill 
%tenant networks' resource requirements.
We also show that \sys can scale to manage large scale multi-tenant data centers hosting hundreds of thousands of 
embedded virtual tenant networks. 
\end{noindlist}

The rest of this paper is organized as follows. In \S \ref{sec:background}, 
we discuss insights that lead to the design choices of \sys. \S \ref{sec:system} 
describes the system design of \sys, and \S\ref{sec:implementation} elaborates 
the implementation of \sys. We evaluate \sys in \S\ref{sec:evaluation}. The related work is 
discussed in \S\ref{sec:related}. \S\ref{sec:conclude} concludes our study.
\fi


==> Managing Recurrent Virtual Network Updates in Multi-Tenant Datacenters A System Perspective/related.tex <==
\section{Related Work and Discussion} \label{sec:related}
%In this section, we briefly discuss related work. 
\parab{Multi-tenancy management.} 
Prior designs for multi-tenant datacenters, 
such as NVP~\cite{vmware} and Netlord~\cite{netlord}, focus on multi-tenancy management 
at hypervisors. For instance, NVP maintains virtual switches on each hypervisor and  
leverages a set of tunnels between each pair of hypervisors to deliver traffic for tenant VMs. 
The actual tenant traffic forwarding in the physical network is not managed. 
Several prior works have considered to perform one-time in-network routing management 
to achieve various goals, such as guaranteed bandwidth \cite{secondnet,predictable,tag}, 
bounded latency \cite{silo,qjump} and user/service isolation \cite{FlowVisor}. 
\sys, instead, focuses on managing \emph{recurrent} routing updates in our production datacenters. 

\parab{A wide variety of performance enhancement.} 
Many approaches have been proposed to improve datacenter networking 
performance. For instance, load balancing approaches \cite{conga, microte, hedera, flare}, 
priority queuing approaches \cite{pdq, pfabric, detail}, 
deadline-aware approaches~\cite{deadline} and DCTCP \cite{dctcp}
are proposed to improve latency performance. Portland~\cite{portland} and fat-tree~\cite{fat-tree} 
propose scalable datacenter architectures to support high bandwidth between servers whereas 
VL2~\cite{vl2} virtualizes datacenters into server pools to allow applications to obtain high throughput.  
Although \sys is not proposed to explicitly improve certain performance, its efficient 
tenant routing management and decoupled design allow network operators to enhance 
a wide variety of \emph{customer-interested} performance metrics, and some of these  
metrics cannot be optimized using prior approaches. 

\parab{Achieving agile routing updates.} To be readily deployable, 
\sys is augmented by SDN to perform agile in-network routing updates. B$4$~\cite{b4} and 
SWAN~\cite{swan} also adopt SDN to perform traffic engineering in wide area 
networks to achieve high inter-datacenter throughput. 




==> Managing Recurrent Virtual Network Updates in Multi-Tenant Datacenters A System Perspective/system.tex <==
\section{System Design} \label{sec:system}
In this section, we elaborate on the design of \sys. 
Figure \ref{fig:system_arch} illustrates the architecture of \sys. 
\sys is built upon a network information 
database and a controller. The network information database 
allows \sys to retrieve network related information, such as network topology and link 
utilization. The controller is used to manage both computation and networking resources, such as 
assigning VMs to tenants and configuring VTNs for tenants. 
\sys's decoupled design is achieved by its VTN embedding module which includes 
routing search engine, routing cache, objective functions and network action container. 

We now describe the workflow of performing routing update using \sys. 
Upon receiving a request, \sys first obtains a list 
of desired routing candidates based on the VM placement. These routing candidates may 
come from either the routing search engine or the routing cache if the VM placement has been 
explored before. Then \sys evaluates each candidate to determine the most desired one 
for achieving a specific goal. To assist evaluation, network operators propose 
evaluation methods, defined as  objective functions, to score each routing candidate. 
The design of objective functions is facilitated  by the global view of all possible routing candidates. 
Further, useful network information (\ie link loads) is retrieved from the network information database. 
Finally, after determining the most desired routing, \sys enforces the VTN embedding inside the network 
by executing network tasks (\ie switch configuration) via the network action container. 
%Afterwards, the VTN embedding request is served and the embedding goal is achieved as well. 


\emph{Although setting up both the 
network information database and the network/computation controller takes considerable 
implementation efforts, we omit these details to focus on the research part of \sys in this paper.} 
Next, we describe each individual component of \sys's VTN embedding module. 
Hereafter, we use \emph{routing} and \emph{VTN} interchangeably to indicate the overlay 
network carrying a tenant's traffic. 



\begin{figure}[t]
  \centering
  \mbox{
    \subfigure{\includegraphics[scale=0.4]{Figures/system_arch.pdf}}
    }
  \caption{The architecture of \sys.}
  \label{fig:system_arch}
\end{figure}
\normalsize

%\subsection{\sys Overview} 

%In a multi-tenant data center, optimizing VTN embeddings is an all-time task on the basis
%of individual tenants, which are up to tens of thousands~\cite{amazon_dc_size,
%amazon_dc_growth}. How to perform one-time VTN embedding might be
%intuitive, however, consistently and frequently
%performing significant amounts of embedding tasks faces scalability concerns.
%Although efficient graph search algorithms, such as Prim's and
%Kruskal's~\cite{prims, kruskals}, have been proposed for years, the overlay network 
%searching cost is still significant due to the large number of optimization
%requests combined from two sides. First, for each newly arrived tenant,
%network operators need to search a virtual network to embed the tenant. Second, 
%the large number of embedded tenants introduce highly dynamic network workload,
%which in turn triggers frequent VTN update requests for the existing
%tenants. 

%Moreover, typically in order to make search process efficient, a greedy
%objective function is applied during search to reduce search space in each
%search iteration. However, finding the optimal routing (\eg lowest latency,
%largest bandwidth or minimal hops) for virtual links is often impossible because
%which physical links will carry which virtual links is uncertain during search. 

%Therefore, \sys adopts a decoupled design in which search is merely based on network
%topology and VM placement whereas optimization is later performed by applying
%objective functions on the routing candidates produced by the search process
%before. As search is not directed by any objective functions, the
%results can be cached and re-used, which saves considerable search efforts. 
%Furthermore, since objective functions are applied afterwards,
%network operators are free to design more sophisticated objective 
%functions (not restricted by greedy ones) to achieve their optimization goals. 
%Further, the objective function is global since operators can have the global view, 
%\eg they are aware of which physical links will serve which virtual links. Therefore, 
%the routing optimality is ensured. 

%Consider the example in Figure \ref{fig:mst}. \sys will
%first find three routing candidates: (b), (c) and (d) in Figure
%\ref{fig:mst}. Then it applies an objective function 
%to determine the optimal overlay to embed the VTN, 
%while knowing the exact mapping between virtual links and physical links.
%Note that in this paper, we use the term ``routing" to indicate the overlay network 
%for the tenant rather than the path between any two VMs or hypervisors. 


%To give the ``illusion" that each tenant is using the whole data center, the host hypervisors perform necessary management such as translating tenant defined addresses to globally routable host addresses via the encapsulations protocols (\eg VXLAN~\cite{vxlan} and NVGRE~\cite{nvgre}). Consequently, as long as the traffic is sent into the network, the operators loss the ability to enforce traffic accountability for each tenant since the tenant traffic is sent on behalf of the physical hosts. 

%There are three four incentives motivate us to decouple search and optimization.

%\comment{high-level of building blocks.}
%In the following, we describe individual components in the system framework of \sys following the optimization workflow (Figure~\ref{fig:system_arch}).

%\subsection{VM Placement as Input}\label{sec:input}
%As discussed in \S\ref{sec:vm_place}, in embedding a tenant network, \sys
%accepts the input as the placement of the tenant's VMs, which is defined as the
%set of hosting hypervisors. While allocating VMs, on the one hand,  
%operators have the incentive to keep the VMs belonging to one tenant local to 
%reduce the networking resources consumption since communication among VMs located within 
%the same hypervisor can be finished within the host. On the other hand, 	 
%VMs fragmentarily distributed across multiple hypervisors are common 
%due to resource constraints on a single hypervisors. 
%Therefore, we expect that 
%each tenant's VMs often span across a few hypervisors, \eg less than $5$.

%Note that we decouples VM placement and VTN embedding is not due 
%to any limitation of \sys, but is because VM placement is often constrained 
%by other factors besides networking performance in practice. 
%We expect that each tenant's VMs often span across a few hypervisors, \eg less than $5$.


\subsection{Routing Search Engine}\label{sec:search_brief}
\iffalse
\begin{figure*}[t]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
    \subfigure{\includegraphics[scale=0.336]{Figures/up_a.pdf}}&
    \subfigure{\includegraphics[scale=0.336]{Figures/up_b.pdf}}&
    \subfigure{\includegraphics[scale=0.336]{Figures/common_node.pdf}}&
    \subfigure{\includegraphics[scale=0.336]{Figures/mst1.pdf}}&
    \subfigure{\includegraphics[scale=0.336]{Figures/mst2.pdf}}\\
\hline
\end{tabular}
\begin{tabularx}{\textwidth}{*5{>{\centering\arraybackslash}X}}
(a) $\texttt{S}_\texttt{1}$'s upward G &
(b) $\texttt{S}_\texttt{3}$'s upward G &
(c) Common nodes &
(d) One ST &
(e) Another ST\\
\end{tabularx}
\caption{Illustrative example for searching routing candidates for hypervisor set [$\texttt{S}_\texttt{1}$,$\texttt{S}_\texttt{3}$,$\texttt{S}_\texttt{4}$]. Part (a) and (b) show the upward graph for $\texttt{S}_\texttt{1}$ and $\texttt{S}_\texttt{3}$, respectively. The upward graph of $\texttt{S}_\texttt{4}$ is omitted. Part (c) shows the common nodes for hypervisor set [$\texttt{S}_\texttt{1}$,$\texttt{S}_\texttt{3}$,$\texttt{S}_\texttt{4}$]. Part (d) and (e) show two routings produced by the search algorithm.} 
\label{fig:search_illu}
\end{figure*}
\fi

Given a certain VM placement, the routing search engine is used to produce a list of \emph{desired} routings 
(or routing candidates). In the typical layered datacenter network layout (\eg 
fattree~\cite{fat-tree}, Clos~\cite{vl2,clos}), a routing is desired if traffic between two VMs does not 
bounce back and forth more than once between two different layers. For random topology (\eg~\cite{jellyfish,SWDC}), 
we can bound the maximum number of hops on VM-pair paths 
to exclude undesired routings. As datacenter fabric is often built with a high level of path redundancy, 
exploring all desired routings will provide sufficient candidates to achieve the embedding goal 
of the routing update request.  
 
 
%Note that it is impossible to find all possible routings for a given VM placement in a network. Instead, the 
%search engine returns all \emph{desired} routings (or routing candidates). 
 
%When receiving VTN embedding requests, \sys first looks up its cache to 
%check if any previous tenants hosted by the same set of hypervisors have been explored
%so that the routing candidates can be re-used. 
%Otherwise, the routing search 
%engine performs graph search to output a list of topology-wise routing candidates. 
%These newly obtained routing candidates will be cached for future use. 
%As analyzed later in \S\ref{sec:benchmark}, the total cache size is ${\sim}100$MB even 
%for a large data center hosting $10$K tenants, which can be easily 
%managed by commodity servers with gigabytes of memory.

%To perform routing search, we expect that \sys retrieves topology related information from a network
%information database. How to design and develop such a network information
%database is out of the scope of this paper as data center operators usually have
%different methodologies to balance the measurement cost and information
%granularity and accuracy. The design of \sys is independent of how the network information database is implemented. 

%Once a request arrives, \sys decides a proper objective function for the corresponding virtual network. Data center operators usually have some pre-defined templates for objective functions, leaving some parameters subject to adjust based on user interests, operator interests, and network dynamics. For example, a valid objective function can be a combination function balancing the weights of latency, bandwidth, and distance, and \sys can tune these weight on-demand. 

%This is the critical step allows us to decouple ``search'' and ``optimization'', which provides several advantages: \first the search results can be re-used repeatedly as long as the network topology remains. In multi-tenant data center, different tenants may end up with the same VM  placement, re-using searching results can save non-trivial cost. \second more than one routing candidate can be offered, which is important as optimization very often is about multiple alternative candidates. \third The decoupling allows the objective function to be more sophisticated. Without decoupling, only greedy objective functions can be applied because only local optimal decisions can be made during search. Objective functions taking into account all links along a path together cannot be coupled into searching. 


%that meets the following requirements. 
%\first The topology consists of a set of isolated zones (or pods), which are 
%inter-connected by several core switches. \second Each pod consists of a few layers. 
%Switches on one layer are connected only to switches on different layers. 
%Most of the common datacenter implementations 
%such as VL2~\cite{vl2} and fat-tree~\cite{fat-tree} satisfy these requirements. 



Next, we propose an algorithm that can produce a comprehensive list 
of all desired routings in layered data center topology. In the network, we associate each node 
with a \emph{height}. All core switches are assigned height 
$1$ and the initial height for other nodes is infinity. Then we trace down from core switches 
towards other nodes to assign them a height. The height of 
a node is the minimum height among all its neighbours plus one. 
All nodes with the same height compose a layer whose layer number is the node height.
We define a path as \emph{straight} if   
all nodes on the path have different heights. 
Straight path is either upward (from a source at a lower layer to a 
destination at a higher layer) or downward. 
%There are two types of straight paths: \emph{upward} and \emph{downward} paths. 
%The upward path is from a source at lower layer to a destination at higher layer. 
%The downward path has the opposite meaning. 
%In Figure \ref{fig:search_illu}, $\texttt{S}_\texttt{1}\texttt{-E}_\texttt{1}\texttt{-A}_\texttt{1}\texttt{-C}_\texttt{1}$ 
%is an upward path and $\texttt{C}_\texttt{1}\texttt{-A}_\texttt{1}\texttt{-E}_\texttt{1}\texttt{-S}_\texttt{1}$ 
%is a downward path. 

%As traffic in desired routings is never forwarded back and forth between different layers. 
In a desired routing, to connect two hypervisors $h_1$ and $h_3$, 
%$\texttt{S}_\texttt{1}$ and $\texttt{S}_\texttt{3}$, 
%$\texttt{S}_\texttt{1}$ 
$h_1$ needs to have a straight path which shares the same endpoint with one of 
%$\texttt{S}_\texttt{3}$'s straight paths. 
$h_3$'s straight paths. 
The shared endpoint is defined as a \emph{common node} for the hypervisor set
%$[\texttt{S}_\texttt{1}$,$\texttt{S}_\texttt{3}]$
$[h_1,h_3]$. Formally, a node is defined as the common node for a set of hypervisors 
%if it has at least one downward path to each hypervisor in the set or equivalently each hypervisor has at least one upward path to reach the node. 
if it has at least one straight path to reach each hypervisor in the set. 
%In Figure \ref{fig:search_illu}, $\texttt{C}_\texttt{1}$ and $\texttt{C}_\texttt{2}$ are common 
%nodes for hypervisor set $[\texttt{S}_\texttt{1}$,$\texttt{S}_\texttt{3}]$. 
%Then flows from $\texttt{S}_\texttt{1}$ can take one upward path to reach one common node (\eg $\texttt{S}_\texttt{1}\texttt{-E}_\texttt{1}\texttt{-A}_\texttt{1}\texttt{-C}_\texttt{1}$) and then bounce back via a downward path 
%from the common node to $\texttt{S}_\texttt{3}$ (\eg $\texttt{C}_\texttt{1}\texttt{-A}_\texttt{3}\texttt{-E}_\texttt{3}\texttt{-S}_\texttt{3}$). 
Then traffic from $h_1$ can first take one straight path to reach the common node and 
then bounces back to reach $h_3$ via another straight path. 
Thus, a routing connecting 
%$[\texttt{S}_\texttt{1}$,$\texttt{S}_\texttt{3}]$ 
$[h_1,h_3]$ is composed of the above two straight paths. Similarly, a routing 
connecting all VMs of a tenant is composed 
of several straight paths, among which each straight path is 
originated from one hypervisor and all these paths are ended at 
one same common node. 

%Based on the algorithm design insight, 
We formulate our search procedure in Algorithm~\ref{algo:search}. 
At the very high level, the algorithm works as follows: \first find all common nodes for the 
hypervisor set (line~\ref{line:common_nodes}); \second for each common node, find one downward straight path 
from the common node to each hypervisor (line~\ref{line:downwardpath}) 
and \third combine these paths to produce one routing candidate (line~\ref{line:combine}). 
Since a routing candidate can only contain one common node (having more will produce loops), 
Algorithm~\ref{algo:search} provably finds all desired routings in the network. 
Even though the algorithm comprehensively finds all desired routings, the algorithm complexity 
is polynomial (not exponential). We defer detailed complexity analysis in \S \ref{sec:appendix}.

\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}
\begin{algorithm}[t]
\SetKwData{GUP}{GetUpwardGraph}
\SetKwData{GetDownwardPath}{GetDownwardPath}
\SetKwData{hs}{hypervisor set}
\SetKwData{cm}{CommonNodes}
\SetKwData{func}{\textbf{Function:}}
\SetKwData{IP}{\textbf{Input:}}
\SetKwData{OP}{\textbf{Output:}}
\footnotesize

\IP VM placement $H$. \\
\OP All desired routing candidates.\\
%\quad All feasible TR candidates for $\mathbf{T}$. \\
\algrule[0.5pt]

	\For{$h_i \in $ \hs $H$}{
		$\mathcal{T}_i \leftarrow$ \GUP{$h_i$}; ~~~$\mathcal{T} \leftarrow \bigcup_{i} \mathcal{T}_i$\; \label{line:upwardgraph}
	}
	\cm $\leftarrow \bigcap_{\mathcal{T}_i \in \mathcal{T}} \mathcal{T}_i$.nodes()\; \label{line:common_nodes}
	\ForEach{$c_j \in$ \cm}{
		\For{$h_i \in$ \hs $H$}{
			$\mathcal{N}_j \leftarrow \bigcup_{i}$ \GetDownwardPath{$c_j,~h_i,~\mathcal{T}_j$}\; \label{line:downwardpath}
		}
	}
	\Return $\mathcal{N} \leftarrow \bigcup_{i} \mathcal{N}_i$\;\label{line:combine}
	
\algrule[0.5pt]

\func \GUP($h_i$) \\ 
\quad \Return The graph containing all upward straight paths starting from $h_i$ and ending 
at core switches.  

\algrule[0.8pt] 

\textbf{\func} \GetDownwardPath{$c_j,~h_i,~\mathcal{T}_j$} \\  
\quad \Return The straight path from $c_j$ to $h_i$ in graph $\mathcal{T}_j$.

\caption{\bf Routing Search Algorithm}\label{algo:search}
\end{algorithm}
\normalsize


For a random data center topology~\cite{jellyfish,SWDC}, \sys can first adopt the $k$-shortest path
algorithm~\cite{shortest} to obtain a set of paths between each hypervisor pair 
and then combine these paths to produce routing candidates. 
$k$ can be parameterized to exclude undesired routings. 
%One concern of \sys's decoupled search and optimization design is that the search cost
%might be non-trivial without applying local objective functions to reduce search
%space, but this is not an issue in practice. Most of the common data center
%designs such as VL2~\cite{vl2,clos} and fat-tree~\cite{fat-tree} organize the
%switches into hierarchical layers, roughly the TOR (edge), the aggregation and
%the core. In such organized and layered network layout, our proposed search
%algorithm (discussed in \S\ref{sec:search}) introduces small costs even if we
%perform exhaustive search for all valid routing candidates in large-scale topologies. 
%For a random network topology (\eg small-world~\cite{smallnet, SWDC} and
%Jellyfish~\cite{jellyfish}), \sys adopts the $k$-shortest path
%algorithm~\cite{k-shortest, new-k-shortest, k-imple} to constrain the size of
%the routing candidates. Note that although \sys may cost more in searching
%embedding options for one VTN, it becomes a wise solution when the volume of
%embedding request grows.

%At this moment, we first focus on the system values of \sys and defer the details about the search algorithm to \S \ref{sec:search}.
%As the focus of this paper is the system values of \sys, we defer the details of our search algorithm to \S \ref{sec:search}. 

\iffalse
\begin{figure}[t]
  \centering
  \mbox{
    \subfigure[Two straight paths.\label{fig:search:a}]{\includegraphics[scale=0.42]{Figures/upward_path.pdf}}\quad
    \subfigure[One VTN candidate.\label{fig:search:b}]{\includegraphics[scale=0.42]{Figures/vtn.pdf}}
    }
  \caption{\footnotesize Search algorithm illustration. Part (a) shows two straight paths starting from \texttt{S1} and \texttt{S3}, respectively. Part (b) shows one routing candidate for a tenant with VM placement \texttt{[S1,S3,S4]}. Note that the topology does not have to be symmetric. }
  \label{fig:search}
\end{figure}
\normalsize
\fi

%We briefly describe the searching algorithm and defer the details in \S \ref{sec:search}. In layered data center topology, we define a path as a \emph{straight} path if all nodes on the path are located in different layers. As illustrated in Figure \ref{fig:search:a}, to allow communication between two hypervisors \texttt{S1} and \texttt{S3}, flows from \texttt{S1} are first sent to \texttt{C1} located in higher layer via the straight path \texttt{S1-E1-A1-C1} and then bounce back to reach \texttt{S3} through another straight path \texttt{C1-A3-E3-S3}. Traffic in layered data centers is never bounced back and forth between two different layers. Thus a routing connecting \texttt{S1} and \texttt{S3} is essentially composed by two straight paths starting from \texttt{S1} and \texttt{S3}, respectively, and ending at the same node (Figure \ref{fig:search:a}). Therefore, by investigating these straight paths from \texttt{S1} and \texttt{S3}, we can construct all the VTN options. Figure \ref{fig:search:b} illustrates one VTN candidate produced by the search algorithm when a tenant's VMs are located in \texttt{S1}, \texttt{S3} and \texttt{S4}.

%Our search algorithm significantly reduces the search space by only exploring the straight paths from each hypervisor rather than the whole graph. Thus, even if we \emph{exhaustively} find all the VTN candidates, the search cost is still acceptable. Table \ref{tab:search_cost} summarizes the search cost (the number of visited edges) for finding all VTN candidates with minimal hops in different fat-tree topologies. We list the number of nodes and edges in the graph under the name of topology to show that the search space is very small compared with whole network size. $\mathcal{N}_v$ is the number of hypervisors one tenant occupies, which is small (\S \ref{sec:vm_place}) in real data center practice. We consider the complexity for both intra-pod (all the hypervisors are located within one pod) and inter-pod (the tenant spans cross at least two pods). For other topologies with larger over-subscription ratio (\eg $2:1$ Clos topology) than fat-tree ($1:1$), the search cost will further be reduced due to the smaller number of redundant paths. 


\subsection{Tenant-Routing Cache}
The search results for routing candidates are cached using a dictionary (hash table) data
structure, where the key is VM placement 
%in terms of a list of hosting hypervisors, 
and the value is a list of all desired routings for the VM placement. 
Each routing is stored as a list of physical link IDs, which can be used to retrieve 
link related information (\eg utilization, status) from the network information database. 
Generally, entries in the dictionary are valid as long as the 
network topology remains the same. In \sys's prototype, 
we associate each entry in the dictionary with a relatively long validation 
period (\eg few weeks), and re-perform routing search after 
an entry is expired. 

In \sys's implementation, we allocate $32$ bits for both the hash key and physical link IDs. 
In \S \ref{sec:evaluation:cache_size}, we show that even in large scale $k{=}32$ fat-tree datacenter 
with over $10$ thousands servers (millions of VMs), the cache size for managing $10$ thousand tenants is 
about $100$ MB, which can be easily managed by commodity servers. 
%Therefore, caching the routing search results can never be a bottleneck in 
%the implementation. 


\subsection{Objective Functions}
The objective functions are used to evaluate routing candidates so as to determine the 
most desired one for fulfilling embedding goals. For instance, a valid
objective function can be as sophisticated as a combination function balancing
latency, bandwidth, the number of hops and so on. Or it can 
be as detailed as optimizing specific virtual links for latency and other virtual 
links for bandwidth. In general, \sys is open to accept any objective function. 
But \sys offers global views on all possible routing candidates so that objective 
functions are not limited to be greedy and local.  Relevant network information, available 
in \sys's network information database, can be applied to evaluate these routing candidates. 
%The ``develop-and-play" design of the objective function module 
%offers complete flexibility to achieve a wide variety of VTN embedding goals.   
By the time of this writing, an instance of \sys deployed in our production datacenter has 
pre-installed tens of abstract objective functions that can be parameterized,  
allowing network operators to achieve a wide variety of VTN embedding goals.  


\subsection{Network Action Container}
After determining the most desired routing, the final step is enforcing the routing 
inside network. The enforcement process is essentially configuring switches on the 
routing (\eg configuring VLAN tags~\cite{vlan} or adding OpenFlow rules~\cite{openflow_spec}) 
to guide the switches to perform desired traffic forwarding.   
To facilitate routing management in large scale datacenters, 
%As some routing configuration actions in our testbed (\eg configure legacy switches) take time, 
we develop a network action container to perform network configurations in a batch. 
For instance, configurations on different ports of one switch are aggregated in 
one thread and configurations on different switches are paralleled via multi-threading. 
As shown in \S \ref{sec:evaluation:switch_config}, the network action container significantly reduces 
the overall configuration latency. 
%One can view the network action container as a plugin to improve \sys's usability. As a flexible 
%system, \sys is open to other plugins that can meliorate the overall system performance and usability. 









